Antigen-Specific Antibody Design via Direct Energy-based Preference Optimization

Antibody design, a crucial task with significant implications across various disciplines such as therapeutics and biology, presents considerable challenges due to its intricate nature. In this paper, we tackle antigen-specific antibody sequence-structure co-design as an optimization problem towards specific preferences, considering both rationality and functionality. Leveraging a pre-trained conditional diffusion model that jointly models sequences and structures of antibodies with equivariant neural networks, we propose direct energy-based preference optimization to guide the generation of antibodies with both rational structures and considerable binding affinities to given antigens. Our method involves fine-tuning the pre-trained diffusion model using a residue-level decomposed energy preference. Additionally, we employ gradient surgery to address conflicts between various types of energy, such as attraction and repulsion. Experiments on RAbD benchmark show that our approach effectively optimizes the energy of generated antibodies and achieves state-of-the-art performance in designing high-quality antibodies with low total energy and high binding affinity simultaneously, demonstrating the superiority of our approach.

==> sections/30-method.tex <==
\begin{figure*}[t]
\begin{center}
\centerline{\includegraphics[width=1.0\textwidth]{figures_compressed_v2/main_figure_compressed_v4.pdf}}
\vspace{-2mm}
\caption{Overview of \method. This process can be summarized as: (a) Generate antibodies with the pre-trained diffusion model; (b) Evaluate the multiple types of residue-level energy and construct preference data; (c) Compute the losses for energy-based preference optimization and mitigate the conflicts between losses of multiple types of energy; (d) Update the diffusion model.% with the merged loss. 
}
\label{fig:illustration}
\vspace{-10mm}
\end{center}
\end{figure*}

\section{Method}



In this section, we present \method, a direct energy-based preference optimization method for designing antibodies with reasonable rationality and functionality (\cref{fig:illustration}). We first define the antibody generation task and introduce the diffusion model for this task in \cref{sec:preliminaries}. 
% Then, we introduce direct residue-level energy-based preference optimization for fine-tuning the diffusion model and analyze its advantages in effectiveness and efficiency in \cref{method:direct_energy_opitmization}. 
Then we introduce residue-level preference optimization for fine-tuning the diffusion model and analyze its advantages in effectiveness and efficiency in \cref{method:direct_energy_opitmization}. 
Finally, in \cref{method:energy_decomposition}, we introduce the energy decomposition and describe how to mitigate the conflicts when optimizing multiple types of energy.


% \dongyu{In \method, we reformulate the antibody design task as an antibody optimization problem with a focus on better rationality and functionality. To achieve the two objectives, we introduce DPO in conjunction with three energy-based rewards, which collectively represent rationality and functionality.}

\subsection{Preliminaries}\label{sec:preliminaries}

We focus on designing CDR-H3 of the antibody given antigen structure as CDR-H3 contributes the most to the diversity and specificity of antibodies \citep{XU200037, AKBAR2021108856} and the rest part of the antibody including the frameworks and other CDRs. Following \citet{DiffAb}, each amino acid is represented by its type $\rs_i\in\{\textsc{ACDEFGHIKLMNPQRSTVWY}\}$, $\text{C}_\alpha$ coordinate $\rvx_i \in \R^3$, and frame orientation $\rmO_i \in \text{SO(3)}$ \citep{kofinas2021rototranslated}, where $i=1,\dots,N$ and $N$ is the number of the amino acids in the protein complex. 
We assume the CDR-H3 to be generated has $m$ amino acids, which can be denoted by $\gR=\{(\rs_j,\rvx_j, \rmO_j) | j=n+1,\dots,n+m\}$, where $n+1$ is the index of the first residue in CDR-H3 sequence. The rest part of the antigen-antibody complex can be denoted by $\gP=\{(\rs_i,\rvx_i,\rmO_i)|i\in\{1,\dots,N\}\backslash\{n+1,\cdots,n+m\}\}$. The antibody generation task can be then formulated as modeling the conditional distribution $P(\gR|\gP)$. 

Denoising Diffusion Probabilistic Model~\citep[DDPM,][]{ddpm} have been introduced to antibody generation by \citet{DiffAb}. This approach consists of a forward \textit{diffusion} process and a reverse \textit{generative} process. The diffusion process gradually injects noises into data as follows:
%{\small
\begin{align*}
    & q(\rs_j^t|\rs_j^{0})=\gC\left( 
    \mathds{1}(\rs_j^{t}) \big|
    \Bar{\alpha}^t \mathds{1}(\rs_j^{0}) + \Bar{\beta}^t \textbf{1} /K
    \right), \\
    & q(\rvx_j^t|\rvx_j^{0})=\gN\left(\rvx_j^t\big| \sqrt{\Bar{\alpha}^t}\rvx_j^{0},\Bar{\beta}^t\mI\right), \\
    & q(\rmO^t_j|\rmO^0_j)=\mathcal{IG}_{\text{SO(3)}}\left(\rmO^t_j|\texttt{ScaleRot}\left(\sqrt{\Bar{\alpha}_t}\rmO^0_j\right),\Bar{\beta}^t\right),
    \label{eq:forward_orientation}
\end{align*}
%\normalsize}
where $(\rs_j^0,\rvx_j^0,\rmO_j^0)$ are the noisy-free amino acid at time step $0$ with index $j$, and $(\rs_j^t,\rvx_j^t,\rmO_j^t)$ are the noisy amino acid at time step $t$. $\{\beta^t\}_{t=1}^T$ is the noise schedule for the diffusion process \citep{ddpm}, and we define $\Bar{\alpha}^t=\prod_{\tau=1}^t(1-\beta^\tau)$ and $\Bar{\beta}^t=1-\Bar{\alpha}^t$. $K$ is the number of amino acid types. Here, $\gC(\cdot)$, $\gN(\cdot)$, and $\mathcal{IG}_{\text{SO(3)}}(\cdot)$ are categorical distribution, Gaussian distribution on $\R^3$, and isotropic Gaussian distribution on SO(3) \citep{leach2022denoising} respectively. \texttt{ScaleRot} scales the rotation angle with fixed rotation axis to modify the rotation matrix \citep{gallier2003computing}.

Correspondingly, the reverse generative process learns to recover data by iterative denoising. The denoising process $p(\gR^{t-1}|\gR^t,\gP)$ from time step $t$ to time step $t-1$ is defined as follows: 
%{\small
\begin{align}
    & p(\rs_j^{t-1}|\gR^t,\gP)=\gC(\rs_j^{t-1}\big| \vf_{\vtheta_1}(\gR^t,\gP)[j]), \\
    & p(\rvx_j^{t-1}|\gR^t,\gP)=\gN(\rvx_j^{t-1}\big| \vf_{\vtheta_2}(\gR^t,\gP)[j], \beta^t\mI), \\
    & p(\rmO_j^{t-1}|\gR^t,\gP)=\mathcal{IG}_{\text{SO(3)}}(\vf_{\vtheta_3}(\gR^t,\gP)[j],\beta^t),
    \label{eq:reverse_orientation}
\end{align}
%\normalsize}
where $\gR^t=\{\rs_j,\rvx_j,\rmO_j\}_{j=l+1}^{l+m}$ is the noisy sequence and structure of CDR-H3 at time step $t$, $\vf_{\vtheta_1},\vf_{\vtheta_2},\vf_{\vtheta_3}$ are parameterized by SE(3)-equivariant neural networks \citep{jing2021learning,jumper2021highly}. $\vf(\cdot)[j]$ denotes the output that corresponds to the $j$-th amino acid. The training objective of the reverse generative process is to minimize the Kullback–Leibler (KL) divergence between variational distribution $p$ and the posterior distribution $q$ as follows:
% {\small
\begin{align}
\label{eq:kl_diffusion}
% \begin{array}{c}
    L=  \mathbb{E}_{\gR^t\sim q}\bigg[ &\frac{1}{m}
    \sum_{j=n+1}^{n+m}\mathbb{D}_{\text{KL}} \Big( q(\gR^{t-1}[j] \vert \gR^{t},\gR^{0},\gP) \big\Vert 
        p_\vtheta (\gR^{t-1}[j]\vert \gR^t,\gP)
    \Big)
    \bigg]. 
% \end{array}
\end{align}
% \normalsize}
With some algebra, we can simplify the above objective and derive the reconstruction loss at time step $t$ as follows:
% {\small
% \begin{align}
%     & \label{eq:kl_s}
%     L^t_{\rs}=\mathbb{E}_{\gR^t}\left[ \sum_{j=l+1}^{l+m} \mathbb{D}_{\text{KL}}
%         \left( 
%             q(s_j^{t-1}|s^t_j,s^0_j) \big\Vert p(s_j^{t-1} | \gR^t,\gP)
%         \right)
%     \right], \\
%     & \label{eq:kl_x}
%     L^t_{\rvx}=\mathbb{E}_{\gR^t}\left[
%         \sum_{j=l+1}^{l+m} \left\Vert \rvx^0_j - \vf_{\theta_2}(\gR^t,\gP) \right\Vert^2
%     \right], \\
%     & \label{eq:kl_o} 
%     L^t_{\rmO} = \mathbb{E}_{\gR^t}\left[ 
%      \sum_{j=l+1}^{l+m} \left\Vert 
%             (\rmO_j^0)^\intercal \vf_{\vtheta_3}(\gR^t,\gP)[j]-\mI
%             \right\Vert^2_F
%     \right].
% \end{align}
% \normalsize}
{\small
\begin{align}
% \setlength{\abovedisplayskip}{0.5pt}
% \setlength{\belowdisplayskip}{0.5pt}
% {\small    
& \begin{aligned}
\small    
\label{eq:kl_s}
    L^t_{\rs}=\mathbb{E}_{\gR^t}  \bigg[ \frac{1}{m} \!\sum_{j=n+1}^{n+m} \!\! \mathbb{D}_{\text{KL}}
        \big( 
            q(\rs_j^{t-1}|\rs^t_j,\rs^0_j) \big\Vert p(\rs_j^{t-1} | \gR^t,\gP)
        \big)
    \bigg]\!, \!\! 
\end{aligned}\\
& \begin{aligned}
\small    
\label{eq:kl_x}
    L^t_{\rvx}=\mathbb{E}_{\gR^t}\bigg[
        \frac{1}{m}
        \sum_{j=n+1}^{n+m} \big\Vert \rvx^0_j - \vf_{\theta_2}(\gR^t,\gP) \big\Vert^2
    \bigg], 
\end{aligned}\\
& \begin{aligned}
\small    
\label{eq:kl_o} 
    L^t_{\rmO} = \mathbb{E}_{\gR^t}\bigg[ 
        \frac{1}{m} \sum_{j=n+1}^{n+m} \big\Vert 
            (\rmO_j^0)^\intercal \vf_{\vtheta_3}(\gR^t,\gP)[j]-\mI
            \big\Vert^2_F
    \bigg],
\end{aligned}
\end{align}
\normalsize}\\
where $\gR^t\sim q(\gR^t|\gR^0)$ and $\gR^0\sim P(\gR|\gP)$, and $\|\cdot\|_F$ is the matrix Frobenius norm.
Note that as \citet{DiffAb} mentioned, \cref{eq:forward_orientation,eq:reverse_orientation} are an empirical perturbation-denosing process instead of a rigorous one. Thus the terminology \textit{KL-divergence} may not be proper for orientation $\rmO$. Nevertheless, we can still approximately derive an empirical reconstruction loss for orientation $\rmO$ as above that works in practice. 
The overall loss is $L\approx\mathbb{E}_{t\sim \text{U}[1,T]}[L^t_\rs+L^t_{\rvx}+L^t_{\rmO}]$. After optimizing this loss, we can start with the noises from the prior distribution and then apply the reverse process to generate antibodies. 

\subsection{Direct Energy-based Preference Optimization}
\label{method:direct_energy_opitmization}

Only the antibodies with considerable sequence-structure rationality and binding affinity can be used as effective therapeutic candidates. Fortunately, these two properties can be estimated by biophysical energy. Thus, we introduce direct energy-based preference optimization to fine-tune the pre-trained diffusion models for antibody design.

% \textcolor{blue}{
% Inspired by DPO~\citep{rafailov2023direct}, we can fine-tune the pre-trained model by pairwise preference data as follows (Note that here we omit the condition $\gP$ for brevity):
% % {\small
% \begin{align*}
% % \label{eq:dpo}
%    \! L_{\text{DPO}} \! = \!\! -\mathbb{E}_{\gR^0_w,\gR^0_l} \! \left[
%     \log\sigma\bigg( 
%         \! \beta\log\! \frac{p_\vtheta(\gR^0_w)}{p_{\text{ref}}(\gR^0_w)} 
%         \!-\! \beta\log\! \frac{p_\vtheta(\gR^0_l)}{p_{\text{ref}}(\gR^0_l)}
%     \! \bigg)
%     \right]\!,\!\!\!
% \end{align*}
% % \normalsize}
% \!where $p_\vtheta$ (resp. $p_{\text{ref}}$) is the distribution induced by the model being fine-tuned (resp. the fixed pre-trained model), $\gR^0_w$ and $\gR^0_l$ are ``winning'' and ``losing'' samples generated by the model, $\beta$ is a hyperparameter that controls regularization. In theory, the above objective is equivalent to the following reward-maximization formulation: 
% \begin{align*}
%     \max_{p_\vtheta} \mathbb{E}_{\gR^0\sim p_{\vtheta}} [r(\gR^0)]-\beta\mathbb{D}_{\text{KL}}(p_\vtheta(\gR^0)\Vert p_{\text{ref}}(\gR^0)).
% \end{align*}
% The antibody with lower energy is preferred, and the reward function $r(\cdot)$ can be defined as negative energy, i.e., $-\gE(\cdot)$.
% }
% \textcolor{red}{
Inspired by RLHF \citep{ouyang2022training}, we can fine-tune the pre-trained model to maximize the reward as: 
\begin{align*}
    \max_{p_\vtheta} \mathbb{E}_{\gR^0\sim p_{\vtheta}} [r(\gR^0)]-\beta\mathbb{D}_{\text{KL}}(p_\vtheta(\gR^0)\Vert p_{\text{ref}}(\gR^0)),
\end{align*}
where $p_\vtheta$ (resp. $p_{\text{ref}}$) is the distribution induced by the model being fine-tuned (resp. the fixed pre-trained model), $\beta$ is a hyperparameter that controls the Kullback–Leibler (KL) divergence regularization. The optimal solution to the above objective takes the form:
\begin{align*}
    p_{\theta^*}(\gR^0)=\frac{1}{Z}p_{\text{ref}}(\gR^0)\exp\Big( \frac{1}{\beta} r(\gR^0) \Big).
\end{align*} 
Following \citet{rafailov2023direct}, we turn to the DPO objective as follows:
\begin{align*}
% \label{eq:dpo}
   \! L_{\text{DPO}} \! = \!\! -\mathbb{E}_{\gR^0_w,\gR^0_l} \! \left[
    \log\sigma\bigg( 
        \! \beta\log\! \frac{p_\vtheta(\gR^0_w)}{p_{\text{ref}}(\gR^0_w)} 
        \!-\! \beta\log\! \frac{p_\vtheta(\gR^0_l)}{p_{\text{ref}}(\gR^0_l)}
    \! \bigg)
    \right]\!,\!\!\!
\end{align*}
where $\sigma(\cdot)$ is sigmoid, $\gR^0_w$ and $\gR^0_l$ are ``winning'' and ``losing'' data pair (i.e., $\gR^0_w\succ\gR^0_l$) sampled from the Bradley-Terry~\citep[BT,][]{bradley1952rank} model with reward $r(\cdot)$, i.e., $p(\gR^0_1\succ\gR^0_2)=\sigma(r(\gR^0_1)-r(\gR^0_2))$. Please refer to \cref{appendix:theoretical_justification} for more detailed derivations.
% }

Due to the intractable $p_\vtheta(\gR^0)$, following \citet{wallace2023diffusion}, we introduce latent variables $\gR^{1:T}$ and utlize the evidence lower bound optimization (ELBO). In particular, $L_{\text{DPO}}$ can be modified as follows:
%\begin{small}
% \vspace{-3.6mm}
\begin{align*}
     & L_{\text{DPO-Diffusion}}= -\mathbb{E}_{\gR^0_w,\gR^0_l}\bigg[ \log\sigma\bigg( 
      \beta \mathbb{E}_{
        \gR^{1:T}_w, \gR^{1:T}_l
     }
     \bigg[ 
        \log \frac{p_\vtheta(\gR^{0:T}_w)}{p_{\text{ref}}(\gR^{0:T}_w)} 
        - \log \frac{p_\vtheta(\gR^{0:T}_l)}{p_{\text{ref}}(\gR^{0:T}_l)}
     \bigg]
     \bigg)\bigg],
\end{align*}
%\end{small}
% \begin{small}
% \begin{align}
%     \begin{array}{c}
%          L_{\text{DPO-Diffusion}}=-\mathbb{E}_{\gR^0_w,\gR^0_l} \log\sigma\Bigg(   \\
%          \left. 
%          \beta \mathbb{E}_{\substack{
%             \gR^{1:T}_w \sim p_{\vtheta}(\gR^{1:T}_w|\gR^0_w)\\
%             \gR^{1:T}_l \sim p_{\vtheta}(\gR^{1:T}_l|\gR^0_l)
%          }}
%          \left[ 
%             \log \frac{p_\vtheta(\gR^{0:T}_w)}{p_{\text{ref}}(\gR^{0:T}_w)} 
%             - \log \frac{p_\vtheta(\gR^{0:T}_l)}{p_{\text{ref}}(\gR^{0:T}_l)}
%          \right]
%          \right).
%     \end{array}
% \end{align}
% \end{small}
where $\gR^{1:T}_w \sim p_{\vtheta}(\gR^{1:T}_w|\gR^0_w)$ and $\gR^{1:T}_l \sim p_{\vtheta}(\gR^{1:T}_l|\gR^0_l)$. 

Following \citet{wallace2023diffusion}, we can utilize Jensen's inequality and convexity of function $-\log\sigma$ to derive the following upper bound of $L_{\text{DPO-Diffusion}}$: 
% \begin{small}
\begin{align*}
     & 
     \Tilde{L}_{\text{DPO-Diffusion}} =-\mathbb{E}_{t,\gR^0_w,\gR^0_l,(\gR^{t-1}_w,\gR^{t}_w),(\gR^{t-1}_l,\gR^{t}_l)}\bigg[\\
     &
       \log\sigma\bigg( \beta T  
        \log \frac{p_\vtheta(\gR^{t-1}_w|\gR^t_w)}{p_{\text{ref}}(\gR^{t-1}_w|\gR^t_w)} %\\
     %& \qquad\qquad
        - 
        \beta T \log \frac{p_\vtheta(\gR^{t-1}_l|\gR^t_l)}{p_{\text{ref}}(\gR^{t-1}_l|\gR^t_l)}
     \bigg)\bigg],
\end{align*}
% \end{small}
% \begin{small}
% \begin{align}
%         \begin{array}{c}
%          L_{\text{DPO-Diffusion}}\leq 
%          \Tilde{L}_{\text{DPO-Diffusion}} =
%          -\mathbb{E}_{\gR^0_w,\gR^0_l\sim p_{\vtheta}(\gR^0)
%          } \log\sigma\\
%           \left(
%          \beta T  
%             \log \frac{p_\vtheta(\gR^{t-1}_w|\gR^t_w)}{p_{\text{ref}}(\gR^{t-1}_w|\gR^t_w)} 
%             - 
%             \beta T \log \frac{p_\vtheta(\gR^{t-1}_l|\gR^t_l)}{p_{\text{ref}}(\gR^{t-1}_l|\gR^t_l)}
%          \right).
%     \end{array}
% \end{align}
% \end{small}
where $t\sim\gU(0,T)$, $(\gR^{t-1}_w,\gR^{t}_w)$ and $(\gR^{t-1}_l,\gR^{t}_l)$ are sampled from reverse generative process of $\gR^0_w$ and $\gR^0_l$, respectively, i.e., $(\gR^{t-1}_w,\gR^{t}_w) \sim p_{\vtheta}(\gR^{t-1}_w,\gR^{t}_w|\gR^0_w)$ and $(\gR^{t-1}_l,\gR^{t}_l) \sim p_{\vtheta}(\gR^{t-1}_l,\gR^{t}_l|\gR^0_l)$.
% \begin{align}
%         \begin{array}{c}
%          L_{\text{DPO-Diffusion}}\leq 
%          \Tilde{L}_{\text{DPO-Diffusion}} \\ =
%          -\mathbb{E}_{
%             \substack{\gR^0_w,\gR^0_l\sim p_{\vtheta}(\gR^0) \\
%                     (\gR^{t-1}_w,\gR^{t}_w) \sim p_{\vtheta}(\gR^{t-1}_w,\gR^{t}_w|\gR^0_w) \\
%                     (\gR^{t-1}_l,\gR^{t}_l) \sim p_{\vtheta}(\gR^{t-1}_l,\gR^{t}_l|\gR^0_l)
%             }
%          } \\
%         \log\sigma  \left(
%          \beta T  
%             \log \frac{p_\vtheta(\gR^{t-1}_w|\gR^t_w)}{p_{\text{ref}}(\gR^{t-1}_w|\gR^t_w)} 
%             - 
%             \beta T \log \frac{p_\vtheta(\gR^{t-1}_l|\gR^t_l)}{p_{\text{ref}}(\gR^{t-1}_l|\gR^t_l)}
%          \right).
%     \end{array}
% \end{align}

In our case, the antibodies with low energy are desired. Thus, we define the reward $r(\cdot)$ as $-\gE(\cdot)/\gT$, where $\gE(\cdot)$ is the energy function and $\gT$ is the temperature. Different from the text-to-image generation where the (latent) reward is assigned to a complete image instead of a pixel \citep{wallace2023diffusion}, we know more fine-grained credit assignment. Specifically, it is known that $\gE(\gR^0)=\sum_{j=n+1}^{n+m}\gE(\gR^0[j])$, i.e., the energy of an antibody is the summation of the energy of its amino acids \citep{ref15}.
Thus the preference can be measured at the residue level instead of the entire CDR level. Besides, we have $\log p_\vtheta(\gR^{t-1}|\gR^{t})=\sum_{j=n+1}^{n+m} \log p_\vtheta(\gR^{t-1}[j]|\gR^{t})$. Thus, by Jensen's inequality and the convexity of $-\log\sigma$, we can further derive the residue-level preference optimization loss, which is an upper bound of $\Tilde{L}_{\text{DPO-Diffusion}}$:
%\begin{small}
\begin{align*}
         &
         L_{\text{residue-DPO-Diffusion}}= -\mathbb{E}_{t,\gR^0_w,\gR^0_l,(\gR^{t-1}_w,\gR^{t}_w),(\gR^{t-1}_l,\gR^{t}_l)}\bigg[ \\ 
         &
         \textstyle{\sum_{j=n+1}^{n+m}}\log\sigma \bigg(\beta T  
            \log \frac{p_\vtheta(\gR^{t-1}_w[j]|\gR^t_w)}{p_{\text{ref}}(\gR^{t-1}_w[j]|\gR^t_w)}    
            - 
            \beta T \log \frac{p_\vtheta(\gR^{t-1}_l[j]|\gR^t_l)}{p_{\text{ref}}(\gR^{t-1}_l[j]|\gR^t_l)}
         \bigg)\bigg].
\end{align*}
%\end{small}
% \begin{align}
%         \begin{array}{c}
%          \Tilde{L}_{\text{DPO-Diffusion}}\leq 
%          L_{\text{EPO}} \\ =
%          -\mathbb{E}_{
%             \substack{\gR^0_w,\gR^0_l\sim p_{\vtheta}(\gR^0) \\
%                     (\gR^{t-1}_w,\gR^{t}_w) \sim p_{\vtheta}(\gR^{t-1}_w,\gR^{t}_w|\gR^0_w) \\
%                     (\gR^{t-1}_l,\gR^{t}_l) \sim p_{\vtheta}(\gR^{t-1}_l,\gR^{t}_l|\gR^0_l)
%             }
%          } \sum_{j=l+1}^{l+m} \\
%         \log\sigma  \left(
%          \beta T  
%             \log \frac{p_\vtheta(\gR^{t-1}_w[j]|\gR^t_w)}{p_{\text{ref}}(\gR^{t-1}_w[j]|\gR^t_w)} 
%             - 
%             \beta T \log \frac{p_\vtheta(\gR^{t-1}_l[j]|\gR^t_l)}{p_{\text{ref}}(\gR^{t-1}_l[j]|\gR^t_l)}
%          \right).
%     \end{array}
% \end{align}
The gradients of $\Tilde{L}_{\text{DPO-Diffusion}}$ and $L_{\text{residue-DPO-Diffusion}}$ w.r.t the parameters $\vtheta$ can be written as:
% \begin{small}
\begin{align*}
      \nabla_\vtheta \Tilde{L}_{\text{DPO-Diffusion}} &=-\beta T \mathbb{E}_{
        t,\gR^{0,t-1,t}_{w,l}\sim p_\vtheta
     }\Big[ \textstyle{\sum_{j=n+1}^{n+m}} \sigma(\Hat{r}(\gR_l^0)-\Hat{r}(\gR_w^0))\\ 
     & 
     \qquad\cdot
     \big(
     \nabla_\vtheta 
        \log p_\vtheta(\gR^{t-1}_w[j]|\gR^t_w)
        - 
       \nabla_\vtheta 
       \log p_\vtheta(\gR^{t-1}_l[j]|\gR^t_l)
     \big)\Big],
\end{align*}
and
\begin{align*}
     \nabla_\vtheta L_{\text{residue-DPO-Diffusion}} &=
      -\beta T \mathbb{E}_{
        t,\gR^{0,t-1,t}_{w,l}\sim p_\vtheta
     }\Big[\textstyle{\sum_{j=n+1}^{n+m}}
     \sigma(\Hat{r}(\gR_l^0[j])-\Hat{r}(\gR_w^0[j]))\\& \qquad \cdot
     \left(
     \nabla_\vtheta 
        \log p_\vtheta(\gR^{t-1}_w[j]|\gR^t_w)
        - 
       \nabla_\vtheta 
       \log p_\vtheta(\gR^{t-1}_l[j]|\gR^t_l)
     \right)\Big],
     % \label{eq:epo_gradient}
\end{align*}
% \end{small}
where $\Hat{r}(\cdot)\coloneqq\log({p_\vtheta(\cdot)}/{p_\text{ref}(\cdot)})$, which can be viewed as the estimated reward by current policy $p_\vtheta$ and $\gR^{0,t-1,t}_{w,l}\sim p_{\vtheta}$ denotes the following for brevity: 
\begin{align*}
    \gR^0_w,\gR^0_l \sim p_{\vtheta}(\gR^0), &&
(\gR^{t-1}_w,\gR^{t}_w) \sim p_{\vtheta}(\gR^{t-1}_w,\gR^{t}_w|\gR^0_w), &&
(\gR^{t-1}_l,\gR^{t}_l) \sim p_{\vtheta}(\gR^{t-1}_l,\gR^{t}_l|\gR^0_l).
\end{align*} 
We can see that $\nabla_\vtheta\Tilde{L}_{\text{DPO-Diffusion}}$ actually reweight $\nabla_\vtheta \log p_\vtheta(\gR^{t-1}[j]|\gR^t)$ with the estimated reward of the complete antibody while $\nabla_\vtheta L_{\text{residue-DPO-Diffusion}}$ does this with the estimated reward of the amino acid itself. 
% Let us take a CDR-H3 with $15$ amino acids whose energy is $[236.0, 25.2, 0.8, \dots, 7.2]$ as an example. The overall energy is $1239.8$, which is usually regarded as a bad candidate. 
In this case, $\nabla_\vtheta\Tilde{L}_{\text{DPO-Diffusion}}$ will increase (resp. decrease) the likelihood of all amino acids of the ``winning'' sample (resp. ``losing'') at the same rate, which may mislead the optimization direction. In contrast, $\nabla_\vtheta L_{\text{residue-DPO-Diffusion}}$ does not have this issue and can fully utilize the residue-level signals from estimated reward to effectively optimize antibodies. 

We further approximate the objective $L_{\text{residue-DPO-Diffusion}}$ by sampling from the forward diffusion process $q$ instead of the reverse generative process $p_\vtheta$ to achieve diffusion-like efficient training. With further replacing $\log \frac{p_\vtheta}{p_{\text{ref}}}$ with $-\log \frac{q}{p_\vtheta} + \log \frac{p_{\text{ref}}}{q}$ which is exactly $-\mathbb{D}_{KL}(q\Vert p_{\vtheta}) + \mathbb{D}_{KL}(q\Vert p_{\text{ref}})$ when taking expectation with respect to $q$, 
% Finally, we can derive the following formula with KL divergence as that in \cref{eq:kl_diffusion}:
we can derive the final loss for fine-tuning the diffusion model as follows:
% \begin{small}
% \begin{align}
% \label{eq:final_epo}
%     \begin{array}{c}
%      L_{\text{\method}} \approx  \Tilde{L}_{\text{residue-DPO-Diffusion}}  \\
%      =  -
%      \mathbb{E}_{
%         \substack{\gR^0_w,\gR^0_l\sim p_{\vtheta}(\gR^0), \gR^{t-1,t}_{w,l} \sim q
%         }
%      } \sum_{j=l+1}^{l+m} 
%      \log\sigma (- \beta T (
%      \\
%      \mathbb{D}_{\text{KL}}(q^{t-1|0,t}_w[j] \Vert p_{\vtheta,w}^{t-1|t}[j])
%     -\mathbb{D}_{\text{KL}}(q^{t-1|0,t}_w [j]\Vert p_{\text{ref},w}^{t-1|t}[j]) 
%     \\
%     -\mathbb{D}_{\text{KL}}(q^{t-1|0,t}_l [j]\Vert p_{\vtheta,l}^{t-1|t}[j])
%     +\mathbb{D}_{\text{KL}}(q^{t-1|0,t}_l[j]\Vert p_{\text{ref},l}^{t-1|t}[j])
%     )
%  ),
% \end{array}
% \end{align}
% \end{small}
% \begin{small}
\begin{align}
\label{eq:final_epo}
    & L_{\text{\method}}=  -
     \mathbb{E}_{t,\gR^0_w,\gR^0_l, (\gR'^{t-1}_w,\gR'^{t}_w),(\gR'^{t-1}_l,\gR'^{t}_l)
     } \Big[ \nonumber
     \\
    & 
     {\sum_{j=n+1}^{n+m}}\log\sigma \Big(
    - \beta T \big\{\mathbb{D}^{w,t}_{\text{KL}}(q  \Vert p_{\vtheta})[j]
    -\mathbb{D}^{w,t}_{\text{KL}}(q \Vert p_{\text{ref}})[j] 
    -\mathbb{D}^{l,t}_{\text{KL}}(q\Vert p_{\vtheta})[j]
    +\mathbb{D}^{l,t}_{\text{KL}}(q\Vert p_{\text{ref}})[j]
    \big\}
 \Big)\Big], 
\end{align}
% \end{small}
where $\gR_w^0$ and $\gR_l^0$ are the ``winning'' and ``losing'' samples generated by the diffusion model, $\gR^0_w,\gR^0_l\sim p_{\vtheta}(\gR)$, $(\gR^{t-1}_w,\gR^{t}_w)$ and $(\gR^{t-1}_l,\gR^{t}_l)$ are sampled from forward diffusion process of $\gR^0_w$ and $\gR^0_l$, respectively, i.e., $(\gR^{t-1}_w,\gR^{t}_w) \sim q(\gR^{t-1}_w,\gR^{t}_w|\gR^0_w)$ and $(\gR^{t-1}_l,\gR^{t}_l) \sim q(\gR^{t-1}_l,\gR^{t}_l|\gR^0_l)$, which can be much more efficient than the reverse generative process that involves hundreds of model forward estimation. Here we use $\mathbb{D}_{\text{KL}}^{w,t}(q\Vert p_\vtheta)[j]$ to denote $\mathbb{D}_{\text{KL}}(q(\gR_w^{t-1}[j]\vert \gR^{t-1},\gR^0)\Vert p_{\vtheta}(\gR^{t-1}_l[j]\vert \gR^0))$. Similar for $\mathbb{D}^{w,t}_{\text{KL}}(q \Vert p_{\text{ref}})[j]$, $\mathbb{D}^{l,t}_{\text{KL}}(q\Vert p_{\vtheta})[j]$, and $\mathbb{D}^{l,t}_{\text{KL}}(q\Vert p_{\text{ref}})[j]$. These KL divergence can be estimated as in \cref{eq:kl_s,eq:kl_x,eq:kl_o}.

\newcommand{\tempcref}[1]{%
  \begingroup
  \hypersetup{allcolors=teal}
  \cref{#1}%
  \endgroup
}

% \begin{algorithm}[tb]
%    \caption{Direct Energy-based Preference Optimization}
%    \label{alg:optimization}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \begin{algorithmic}
%    \REQUIRE pre-trained diffusion model parameter $\vtheta$, the antigen-antibody complex except CDR-H3 $\gP$, the number of iterations $N_{\text{outer}}$, the number of optimization steps per iteration $N_{\text{inner}}$ sampling batch size $B_{\text{sample}}$, training batch size $B_{\text{train}}$, energy functions and their weights $\{(\gE_v(\cdot), w_v)\}_{v=1}^V$, learning rate $\eta$
%    \ENSURE model parameters $\vtheta$, generated antibodies set $\gD$
%    \STATE $\gD \gets \emptyset; \vtheta_{\text{ref}}\gets \vtheta$
%    \FOR{$\tau=1$  {\bfseries to} $N_{\text{outer}}$}
%    \STATE \textcolor{teal}{\# Sample $B_{\text{sample}}$ antibodies.}
%    \STATE $\{\gR_i\} \gets \texttt{Generate}(\vtheta, \gP, B_{\text{sample}})$
%    \STATE \textcolor{teal}{\# Evaluate the residue-level energy.}
%    \STATE $\{ \{\gE_v(\gR_i)[j]\}_{j=l+1,v=1}^{l+m,V} \} \gets \texttt{Evaluate}(\{\gR_i\})$
%    \STATE \textcolor{teal}{\# Append to the dataset.}
%    \STATE $\gD\gets \gD\cup \{ \{(\gR_i,\gE_v(\gR_i)[j]\}_{j=l+1,v=1}^{l+m,V}) \}$
%         \FOR{$\nu=1$ {\bfseries to} $N_{\text{outer}}$}
%         \STATE \textcolor{teal}{\# Randomly construct $B_{\text{train}}$ pairs of antibodies.}
%         \STATE $\{(\gR_w, \gR_l)_i\}\gets \texttt{SamplePairBatch}(\gD,B_{\text{train}})$
%         \STATE \textcolor{teal}{\# Compute \method loss as \tempcref{eq:final_epo}.}
%         \STATE $\{{L}_v\} \gets \texttt{ComputeEPOLoss}(\{(\gR_w, \gR_l)_i\},\vtheta,\vtheta_{\text{ref}})$
%         \STATE \textcolor{teal}{\# Apply gradient surgery as \tempcref{eq:pcgrad}.}
%         \STATE $\{\nabla_{\vtheta} L_v\}\gets \texttt{GradientSurgery}(\{\nabla_{\vtheta} L_v\})$ 
%         \STATE \textcolor{teal}{\# Update model parameters.}
%         \STATE $\vtheta\gets \vtheta-\eta \sum_{v=1}^V w_v \nabla_{\vtheta}L_v$
%         \ENDFOR
%    \ENDFOR
% \end{algorithmic}
% \end{algorithm}

\subsection{Energy Decomposition and Conflict Mitigation}
\label{method:energy_decomposition}

The energy usually consists of different types, such as attraction and repulsion. Empirically, direct optimization on \dongyu{single} energy will lead to some undesired ``shortcuts''. Specifically, in some cases, repulsion dominates the energy of the antibody so the model will push antibodies as far from the antigen as possible to decrease the repulsion during optimization, and finally fall into a bad local minima. This effectively reduces the repulsion, but also completely eliminates the attraction between antibodies and antigens, which seriously impairs the functionality of the antibody. This motivates us to explicitly express the energy with several distinct terms and then control the optimization process towards our preference.  

Inspired by \citet{yu2020gradient}, we utilize ``gradient surgery'' to alleviate interference between different types of energy during energy preference optimization. More specifically, we have $\gE(\cdot)=\sum_{v=1}^V w_v \gE_v(\cdot)$, where $V$ is the number of types of energy, and $w_v$ is a constant weight for the $v$-th kind of energy. For each type of energy $\gE_v(\cdot)$, we compute its corresponding energy preference gradient $\nabla_\vtheta L_v$ as \cref{eq:final_epo}, and then alter the gradient by projecting it onto the normal plane of the other gradients (in a random order) if they have conflicts. This process works as follows:
\begin{align}
    \nabla_\vtheta L_v \leftarrow \nabla_\vtheta L_v -\frac{\min{(\nabla_\vtheta L_v^\top \nabla_\vtheta L_u,0)}}{\left\Vert\nabla_\vtheta L_u\right\Vert^2} \nabla_\vtheta L_u,
    \label{eq:pcgrad}
\end{align}
where $v \in \{1,\dots,V \}$ and $u=\texttt{Shuffle}(1,\dots,V)$. 

%The complete direct energy-based preference optimization process can be summarized as \cref{alg:optimization}.


% \newcommand{\tempcref}[1]{%
%   \begingroup
%   \hypersetup{allcolors=teal}
%   \cref{#1}%
%   \endgroup
% }

% \begin{algorithm}[tb]
%    \caption{Direct Energy-based Preference Optimization}
%    \label{alg:optimization}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \begin{algorithmic}
%    \REQUIRE pre-trained diffusion model parameters $\vtheta$, the antigen-antibody complex except CDR-H3 $\gP$, the number of iterations $N_{\text{outer}}$, the number of optimization steps per iteration $N_{\text{inner}}$ sampling batch size $B_{\text{sample}}$, training batch size $B_{\text{train}}$, energy functions and their weights $\{(\gE_v(\cdot), w_v)\}_{v=1}^V$, learning rate $\eta$
%    \ENSURE model parameters $\vtheta$, generated antibodies set $\gD$
%    \STATE $\gD \gets \emptyset; \vtheta_{\text{ref}}\gets \vtheta$
%    \FOR{$\tau=1$  {\bfseries to} $N_{\text{outer}}$}
%    \STATE \textcolor{teal}{\# Sample $B_{\text{sample}}$ antibodies.}
%    \STATE $\{\gR_i\} \gets \texttt{Generate}(\vtheta, \gP, B_{\text{sample}})$
%    \STATE \textcolor{teal}{\# Evaluate the residue-level energy.}
%    \STATE $\{ \{\gE_v(\gR_i)[j]\}_{j=l+1,v=1}^{l+m,V} \} \gets \texttt{Evaluate}(\{\gR_i\})$
%    \STATE \textcolor{teal}{\# Append to the dataset.}
%    \STATE $\gD\gets \gD\cup \{ \{(\gR_i,\gE_v(\gR_i)[j]\}_{j=l+1,v=1}^{l+m,V}) \}$
%         \FOR{$\nu=1$ {\bfseries to} $N_{\text{outer}}$}
%         \STATE \textcolor{teal}{\# Randomly construct $B_{\text{train}}$ pairs of antibodies.}
%         \STATE $\{(\gR_w, \gR_l)_i\}\gets \texttt{SamplePairBatch}(\gD,B_{\text{train}})$
%         \STATE \textcolor{teal}{\# Compute \method loss as \tempcref{eq:final_epo}.}
%         \STATE $\{{L}_v\} \gets \texttt{ComputeEPOLoss}(\{(\gR_w, \gR_l)_i\},\vtheta,\vtheta_{\text{ref}})$
%         \STATE \textcolor{teal}{\# Apply gradient surgery as \tempcref{eq:pcgrad}.}
%         \STATE $\{\nabla_{\vtheta} L_v\}\gets \texttt{GradientSurgery}(\{\nabla_{\vtheta} L_v\})$ 
%         \STATE \textcolor{teal}{\# Update model parameters.}
%         \STATE $\vtheta\gets \vtheta-\eta \sum_{v=1}^V w_v \nabla_{\vtheta}L_v$
%         \ENDFOR
%    \ENDFOR
% \end{algorithmic}
% \end{algorithm}

==> sections/60-impact.tex <==
\section*{Impact Statements}
Our work on antibody design can be used in developing potent therapeutic antibodies and accelerate the research process of drug discovery. Our method may be adapted to other scenarios of computer-aided design, such as small molecule design, material design, and chip design.  It is also needed to ensure the responsible use of our method and refrain from using it for harmful purposes.

==> sections/checklist.tex <==

\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}



==> sections/checklist_update.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The main claims made in the abstract and introduction accurately reflect the paper's contributions and scope.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discusses the limitations of the work in \cref{appendix:limitations_and_future_work}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides the full set of assumptions and a complete (and correct) proof for each theoretical result.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper fully discloses all the information needed to reproduce the main experimental results of the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The release of code requires approval.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper specifies all the training and test details in \cref{appendix:training_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We lack sufficient computing power to complete such statistical tests.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper provides sufficient information on the computer resources.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conducted in the paper conforms, in every respect, with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discusses both positive and negative impacts of the work performed in \cref{appendix:impact_statements}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The creators or original owners of assets (e.g., code, data, models), used in the paper, are properly credited.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> tables/aar_rmsd.tex <==
% \renewcommand{\arraystretch}{1.}
\begin{tabular}{lcc}
\hline
Methods                & AAR  & RMSD  \\ \hline
HERN                   & 33.17\% & 9.86 \\
MEAN                   & 33.47\% & 1.82 \\
dyMEAN                 & 40.95\% & 7.24 \\
DiffAb                 & 36.71\% & 2.13 \\
\method                & 26.43\% & 2.43 \\ \hline
\end{tabular}
% \renewcommand{\arraystretch}{1}

==> tables/aar_rmsd_all.tex <==
\noindent
\begin{minipage}{.32\linewidth}
\centering
%\captionof{table}{Original}
\begin{tabular}{lll}
\hline
Method & AAR     & RMSD \\ \hline
HERN   & 33.17\% & 9.86 \\
MEAN   & 33.47\% & 1.82 \\
dyMEAN & 40.95\% & 7.24 \\
DiffAb & 36.42\% & 2.34 \\
\method  & 26.46\% & 2.48 \\ \hline
\end{tabular}
\end{minipage}%
\begin{minipage}{.32\linewidth}
\centering
%\captionof{table}{rank1}
\begin{tabular}{lll}
\hline
Method & AAR     & RMSD \\ \hline
HERN   & 22.35\% & 9.79 \\
MEAN   & 35.95\% & 1.92 \\
dyMEAN & 41.95\% & 7.31 \\
DiffAb & 36.77\% & 2.14 \\
\method  & 26.46\% & 2.48 \\ \hline
\end{tabular}
\end{minipage}%
\begin{minipage}{.32\linewidth}
\centering
%\captionof{table}{full}
\begin{tabular}{lll}
\hline
Method & AAR     & RMSD \\ \hline
HERN   & 24.79\% & 9.78 \\
MEAN   & 36.24\% & 1.97 \\
dyMEAN & 41.28\% & 7.31 \\
DiffAb & 36.52\% & 2.47 \\
\method  & 25.95\% & 2.77 \\ \hline
\end{tabular}
\end{minipage}

==> tables/ablation_sft.tex <==
\renewcommand{\arraystretch}{1.}
\begin{tabular}{l|cc|cc}
\toprule
% \diagbox{Model}{Metric} 
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{CDR $E_{\text{total}}$ ($\downarrow$)} & \multicolumn{2}{c}{CDR-Ag $\Delta G$ ($\downarrow$)}   \\
 & Avg. & Med. & Avg. & Med.   \\
\midrule
% Reference & \multicolumn{2}{c|}{62.28} & \multicolumn{2}{c}{4.72}   \\
Reference & 62.28 & 62.28 & -4.72 & -4.72   \\
\midrule
DiffAb     & 288.10 & 289.81 & 0.84 & -1.03  \\
$\text{DiffAb}_{\text{SFT}}$    & 274.01 & 281.47  & -2.72 & -2.65  \\
\method & \textbf{88.15} & \textbf{85.13} & \textbf{-2.97} & \textbf{-2.66}  \\
\bottomrule
\end{tabular}
\renewcommand{\arraystretch}{1}

==> tables/all_complexes_revision_avg.tex <==
{\tiny
% Reduce the font size
\setlength{\tabcolsep}{2pt} % Reduce the column separation
% \renewcommand{\arraystretch}{1.2}

\begin{longtable}{c|rrrr|rrrr|rrrr|rrrr|rrrr|rrrr|rrrr}
\caption{Detailed evaluation results for reference antibodies and average evaluation results for antibodies designed by HERN, MEAN, dyMEAN, DiffAb, \method, and \methodp for 55 antigens. The data source is the same as that in \cref{tab:main_result}. For simplicity, we use A, B, C, and D to stand for CDR $E_{\text{total}}$, CDR-Ag $\Delta G$, PHR, and pLL respectively in this table. The unit is kcal/mol and omitted for brevity.}\label{tab:all_complexes_avg}
\endfirsthead
\endhead
\toprule
% \diagbox{Model}{Metric} 


\multirow{2}{*}{\textbf{PDB id}} 
& \multicolumn{4}{c|}{\textbf{RAbD (Reference)}}
& \multicolumn{4}{c|}{\textbf{HERN}}
 & \multicolumn{4}{c|}{\textbf{MEAN}}
  & \multicolumn{4}{c|}{\textbf{dyMEAN}}
  & \multicolumn{4}{c|}{\textbf{DiffAb}}
    & \multicolumn{4}{c|}{\textbf{\method}}
        & \multicolumn{4}{c}{\textbf{\methodp}}
\\
% & CDR & $E_{\text{nonRep}}$ & $E_{\text{Rep}}$ &  $\Delta G$ & CDR & CDR-Ag & CDR-Ag & CDR-Ag& CDR & CDR-Ag & CDR-Ag & CDR-Ag& CDR & CDR-Ag & CDR-Ag & CDR-Ag& CDR & CDR-Ag & CDR-Ag & CDR-Ag& CDR & CDR-Ag & CDR-Ag & CDR-Ag \\
% & & Rep & nonRep & Total & & Rep & nonRep & Total & & Rep & nonRep & Total & & Rep & nonRep & Total & & Rep & nonRep & Total & & Rep & nonRep & Total\\
& A&B&C&D& A&B&C&D& A&B&C&D& A&B&C&D& A&B&C&D & A&B&C&D& A&B&C&D\\
\midrule
1a14 & 62.28 & -4.72 & 40.00\% & -1.56 & 5084.28 & 163.75 & 40.87\% & -1.57 & 7614.74 & 280.22 & 31.60\% & -1.66 & 5284.77 & 187.78 & 37.71\% & -1.93 & 1314.20 & 534.21 & 31.35\% & -1.86 & 336.02 & 88.64 & 76.84\% & -2.06 & 800.86 & 334.38 & 36.28\% & -1.78 \\
1a2y & -22.18 & -4.81 & 20.00\% & -1.30 & 8082.04 & 236.89 & 42.08\% & -1.27 & 3722.91 & 75.93 & 35.31\% & -1.22 & 70.82 & -0.04 & 60.00\% & -1.15 & 538.97 & 50.06 & 37.19\% & -1.71 & 247.86 & 9.25 & 48.18\% & -1.93 & 428.22 & 50.79 & 26.61\% & -1.74 \\ 
1fe8 & 25.79 & -14.84 & 44.44\% & -2.61 & 4920.00 & 6.17 & 42.48\% & -2.15 & 3914.47 & 885.65 & 28.82\% & -1.57 & 909.90 & 255.99 & 55.21\% & -1.89 & 1239.61 & 600.91 & 45.66\% & -2.24 & 880.26 & 257.83 & 48.49\% & -2.43 & 1010.34 & 382.26 & 35.99\% & -2.31 \\ 
1ic7 & 19.96 & -2.62 & 57.14\% & -2.89 & 8868.32 & 115.08 & 41.37\% & -1.84 & 1694.93 & 59.31 & 25.67\% & -1.98 & 589.59 & 144.47 & 42.86\% & -1.45 & 665.83 & 102.33 & 48.07\% & -1.75 & 236.16 & 11.19 & 85.19\% & -1.88 & 318.16 & 36.02 & 51.34\% & -1.48 \\ 
1iqd & 43.36 & -5.47 & 70.00\% & -2.66 & 10278.46 & 281.72 & 43.07\% & -2.29 & 4922.51 & 684.45 & 52.14\% & -1.75 & 861.34 & 921.96 & 59.64\% & -1.97 & 1277.45 & 1218.19 & 49.58\% & -2.36 & 291.91 & 73.22 & 79.27\% & -2.15 & 744.88 & 686.06 & 63.91\% & -2.24 \\ 
1n8z & 41.88 & -8.00 & 53.85\% & -2.50 & 7478.36 & 143.92 & 38.98\% & -2.15 & 5909.10 & 773.06 & 28.57\% & -1.78 & 2623.55 & 182.40 & 53.85\% & -2.05 & 1366.55 & 875.67 & 36.78\% & -2.16 & 522.38 & 158.66 & 65.10\% & -2.28 & 983.06 & 591.70 & 38.94\% & -2.13 \\ 
1ncb & 29.72 & -11.94 & 38.46\% & -2.35 & 15891.62 & 1045.70 & 39.66\% & -1.94 & 7830.64 & 2181.26 & 19.63\% & -1.51 & 7676.52 & 5373.85 & 32.33\% & -2.15 & 2757.11 & 2413.60 & 37.78\% & -2.19 & 1226.72 & 597.29 & 68.07\% & -2.24 & 2307.18 & 1598.22 & 45.27\% & -2.14 \\ 
1osp & -1.39 & -15.94 & 42.86\% & -1.78 & 22779.04 & 39545.20 & 40.10\% & -2.21 & 7299.27 & 2093.95 & 40.33\% & -1.93 & 10450.61 & 14898.46 & 40.29\% & -2.34 & 1726.43 & 1163.36 & 38.39\% & -2.33 & 741.85 & 281.07 & 64.96\% & -2.27 & 1354.85 & 393.58 & 35.34\% & -2.13 \\ 
1uj3 & -12.93 & -11.45 & 40.00\% & -2.16 & 12931.58 & 24.87 & 43.54\% & -2.22 & 3651.92 & 833.83 & 26.09\% & -1.46 & 725.91 & 60.68 & 59.69\% & -1.66 & 1201.06 & 515.24 & 46.46\% & -2.25 & 548.70 & 309.96 & 60.94\% & -2.50 & 902.98 & 535.91 & 40.94\% & -2.12 \\ 
1w72 & 8.36 & -16.06 & 46.67\% & -2.05 & 13064.14 & 236.14 & 38.19\% & -1.97 & 9270.47 & 359.62 & 29.31\% & -1.66 & 4646.75 & 1691.72 & 32.78\% & -2.27 & 1898.70 & 2301.58 & 46.77\% & -2.10 & 541.99 & 323.45 & 79.17\% & -1.86 & 1475.37 & 1319.43 & 45.63\% & -1.82 \\ 
2adf & -20.47 & -15.53 & 36.36\% & -2.16 & 9963.24 & 668.11 & 41.43\% & -2.11 & 5242.10 & 1284.62 & 30.30\% & -1.90 & 1265.15 & 737.82 & 51.33\% & -1.79 & 2119.86 & 2177.12 & 35.89\% & -2.37 & 1211.16 & 1125.38 & 49.15\% & -2.42 & 1863.22 & 1872.10 & 31.91\% & -2.32 \\ 
2b2x & 5.41 & -0.90 & 58.33\% & -2.22 & 10070.26 & 1046.74 & 41.10\% & -2.16 & 10872.33 & 92.94 & 18.79\% & -1.89 & 4030.74 & 2568.95 & 26.13\% & -1.52 & 1572.54 & 348.72 & 44.23\% & -2.16 & 627.10 & 120.47 & 76.78\% & -2.15 & 1033.04 & 272.63 & 47.01\% & -1.93 \\ 
2cmr & 5.25 & -9.79 & 41.67\% & -2.20 & 15455.06 & 1146.95 & 42.49\% & -2.24 & 6012.22 & 1194.67 & 26.30\% & -1.82 & 3176.59 & 1049.25 & 50.00\% & -1.78 & 2254.27 & 1702.79 & 49.39\% & -2.18 & 1493.98 & 908.39 & 54.64\% & -1.96 & 1670.16 & 1134.01 & 42.45\% & -1.84 \\ 
2dd8 & 68.27 & -7.21 & 63.64\% & -2.27 & 10822.48 & 1265.56 & 41.95\% & -2.14 & 6360.61 & 261.43 & 22.25\% & -1.62 & 1868.70 & 1084.35 & 53.98\% & -1.55 & 921.64 & 114.18 & 50.00\% & -2.15 & 304.55 & 11.63 & 65.30\% & -2.03 & 435.60 & 49.50 & 54.50\% & -2.04 \\ 
2vxt & -10.32 & -12.95 & 66.67\% & -1.76 & 5017.31 & -0.53 & 46.18\% & -2.20 & 1378.61 & 198.35 & 16.93\% & -1.99 & 230.60 & 170.56 & 50.00\% & -1.11 & 1286.01 & 1211.78 & 51.22\% & -1.99 & 378.06 & 127.33 & 87.76\% & -2.11 & 523.04 & 303.94 & 67.54\% & -1.62 \\ 
2xqy & -3.67 & -16.14 & 54.55\% & -2.68 & 11783.79 & 112.94 & 41.34\% & -2.07 & 4532.76 & 633.59 & 35.23\% & -1.38 & 1831.64 & 1248.24 & 45.45\% & -0.76 & 975.16 & 576.50 & 35.32\% & -2.18 & 521.87 & 171.23 & 57.48\% & -2.08 & 1093.36 & 508.48 & 35.79\% & -2.17 \\ 
2xwt & -19.96 & -27.99 & 50.00\% & -2.57 & 14800.89 & 1547.70 & 38.63\% & -2.11 & 6877.42 & 3150.51 & 25.65\% & -1.55 & 4033.71 & 4267.90 & 42.66\% & -2.19 & 1941.55 & 1394.53 & 42.19\% & -2.11 & 279.27 & 40.72 & 80.77\% & -2.12 & 900.33 & 356.91 & 52.69\% & -1.94 \\ 
2ypv & 4.72 & -6.94 & 25.00\% & -1.43 & 17470.94 & 1153.82 & 40.49\% & -2.12 & 5817.70 & 2291.43 & 27.82\% & -1.48 & 5638.27 & 6442.33 & 30.99\% & -1.25 & 2312.54 & 2615.65 & 37.98\% & -2.13 & 409.78 & 151.56 & 83.33\% & -2.24 & 1161.97 & 598.35 & 49.83\% & -2.06 \\ 
3bn9 & 81.92 & -0.89 & 33.33\% & -1.71 & 12219.73 & 904.99 & 43.23\% & -2.24 & 4956.22 & 92.90 & 26.50\% & -2.24 & 8516.00 & 0.20 & 66.67\% & -1.91 & 1911.65 & 261.66 & 49.13\% & -2.32 & 717.15 & 46.78 & 77.90\% & -2.53 & 1086.68 & 172.95 & 38.04\% & -2.30 \\ 
3cx5 & -18.25 & -14.91 & 33.33\% & -1.80 & 18070.35 & 1402.27 & 39.48\% & -1.46 & 6987.09 & 303.81 & 38.54\% & -1.55 & 5257.45 & 62.91 & 35.45\% & -1.26 & 1652.10 & 421.00 & 38.65\% & -1.84 & 388.32 & 89.93 & 74.93\% & -1.81 & 923.14 & 235.49 & 44.65\% & -1.80 \\ 
3ffd & 43.13 & -12.63 & 36.36\% & -2.39 & 3076.25 & 542.93 & 42.19\% & -2.05 & 2685.49 & 527.96 & 40.48\% & -1.55 & 576.62 & 741.54 & 54.55\% & -1.76 & 1306.04 & 1877.71 & 42.80\% & -2.06 & 621.94 & 694.12 & 46.64\% & -2.30 & 872.12 & 1078.66 & 33.99\% & -2.11 \\ 
3hi6 & -1.47 & -12.35 & 46.15\% & -1.93 & 13361.85 & 68.13 & 39.62\% & -1.99 & 11746.52 & 6383.11 & 22.16\% & -1.95 & 3042.84 & 2664.46 & 55.01\% & -2.03 & 2603.22 & 3406.63 & 47.36\% & -2.14 & 1347.67 & 1059.13 & 65.30\% & -2.07 & 1722.26 & 1465.23 & 43.35\% & -1.91 \\ 
3k2u & 18.71 & -14.57 & 72.73\% & -3.02 & 11409.01 & 28.71 & 41.38\% & -2.09 & 6503.22 & 2403.08 & 24.86\% & -1.59 & 988.56 & 1328.85 & 54.55\% & -1.33 & 1034.26 & 1211.08 & 39.91\% & -2.05 & 417.15 & 228.56 & 57.20\% & -2.05 & 830.86 & 595.22 & 33.55\% & -1.97 \\ 
3l95 & -1.18 & -18.48 & 58.33\% & -2.50 & 15605.61 & 371.11 & 41.02\% & -2.09 & 6733.72 & 1246.90 & 24.83\% & -1.91 & 1090.77 & 529.55 & 66.49\% & -1.49 & 1164.38 & 767.77 & 40.84\% & -2.03 & 447.80 & 95.36 & 70.62\% & -1.90 & 817.12 & 251.49 & 51.82\% & -1.83 \\ 
3mxw & -7.55 & -19.04 & 41.67\% & -2.10 & 7969.63 & 726.31 & 37.63\% & -1.91 & 6335.74 & 805.41 & 31.90\% & -2.49 & 4070.17 & 1968.18 & 33.33\% & -1.90 & 1610.09 & 1589.86 & 39.11\% & -2.09 & 251.53 & 157.53 & 76.52\% & -2.44 & 652.83 & 664.27 & 48.61\% & -2.08 \\ 
3nid & -21.55 & -28.54 & 41.67\% & -2.06 & 10711.38 & 702.13 & 42.75\% & -2.08 & 9531.63 & 3817.14 & 21.96\% & -2.18 & 1542.49 & 1474.66 & 55.16\% & -1.89 & 2327.91 & 3134.96 & 34.81\% & -2.14 & 1567.97 & 1795.32 & 55.56\% & -2.29 & 2246.97 & 2987.74 & 34.16\% & -2.15 \\ 
3o2d & 0.23 & -13.42 & 46.67\% & -2.01 & 7277.36 & 1747.32 & 39.24\% & -1.82 & 9294.13 & 231.91 & 29.31\% & -1.86 & 3792.46 & 238.21 & 36.74\% & -1.64 & 1968.51 & 671.50 & 37.50\% & -2.14 & 590.40 & 52.58 & 77.71\% & -2.38 & 1270.30 & 270.11 & 46.28\% & -2.01 \\ 
3rkd & -6.61 & -10.35 & 43.75\% & -1.94 & 4874.78 & 419.59 & 37.37\% & -2.11 & 5400.31 & 177.87 & 53.58\% & -1.98 & 2224.89 & 28.81 & 37.63\% & -2.18 & 2545.63 & 1419.63 & 38.77\% & -2.15 & 388.75 & 39.36 & 69.63\% & -2.57 & 1140.76 & 205.51 & 34.64\% & -2.09 \\ 
3s35 & -4.63 & -5.60 & 20.00\% & -2.23 & 9079.72 & 410.94 & 44.32\% & -2.03 & 3690.15 & 903.86 & 23.33\% & -1.62 & 1052.31 & 1200.26 & 57.19\% & -1.30 & 1228.31 & 1383.63 & 38.70\% & -1.99 & 185.90 & 86.67 & 77.55\% & -2.14 & 244.30 & 106.91 & 64.01\% & -1.92 \\ 
3w9e & -9.93 & -18.41 & 40.00\% & -2.29 & 18322.87 & 2687.04 & 39.72\% & -1.98 & 9415.71 & 2837.23 & 23.68\% & -2.00 & 9644.55 & 13212.83 & 40.00\% & -2.16 & 1768.13 & 1320.91 & 45.38\% & -2.18 & 1266.82 & 426.19 & 57.95\% & -2.08 & 1807.16 & 814.79 & 35.35\% & -1.97 \\ 
4cmh & -19.18 & -16.54 & 30.77\% & -1.63 & 9638.37 & 409.93 & 38.86\% & -1.95 & 11848.30 & 1885.29 & 26.96\% & -2.10 & 5226.83 & 1468.30 & 30.77\% & -1.95 & 2710.24 & 2869.13 & 41.79\% & -2.00 & 646.94 & 637.58 & 82.17\% & -1.97 & 2091.31 & 1976.46 & 45.95\% & -1.88 \\ 
4dtg & 7.56 & -5.43 & 50.00\% & -2.31 & 12267.42 & 20920.65 & 38.91\% & -1.90 & 5047.79 & 1.41 & 52.72\% & -1.71 & 1969.31 & 965.74 & 44.68\% & -1.88 & 1753.12 & 1906.32 & 37.98\% & -2.09 & 195.38 & 67.03 & 87.13\% & -2.09 & 913.31 & 826.23 & 45.76\% & -2.02 \\ 
4dvr & -6.74 & 1.13 & 66.67\% & -2.89 & 11025.32 & 16.41 & 39.06\% & -2.10 & 4932.19 & 89.35 & 39.63\% & -1.52 & 3080.76 & 972.57 & 33.46\% & -2.57 & 860.12 & 339.55 & 38.50\% & -2.19 & 212.96 & 78.48 & 67.27\% & -2.47 & 474.54 & 235.55 & 40.15\% & -2.25 \\ 
4ffv & 28.69 & 0.67 & 50.00\% & -2.96 & 3822.72 & 164.84 & 43.91\% & -1.96 & 2064.08 & 53.98 & 20.89\% & -1.62 & 517.77 & -0.47 & 69.95\% & -1.48 & 712.45 & 71.58 & 38.96\% & -1.87 & 247.26 & 0.49 & 73.39\% & -1.78 & 462.92 & 15.58 & 53.49\% & -1.69 \\ 
4fqj & 33.50 & -21.93 & 38.89\% & -1.66 & 16862.12 & 308.56 & 40.08\% & -2.08 & 6404.03 & 1009.16 & 38.77\% & -2.20 & 7140.47 & 993.46 & 41.23\% & -2.04 & 3534.93 & 3314.58 & 40.10\% & -2.15 & 1675.57 & 703.82 & 70.95\% & -2.36 & 2682.46 & 1371.78 & 36.75\% & -2.00 \\ 
4g6j & 0.30 & -8.81 & 45.45\% & -1.92 & 11113.87 & 720.86 & 42.42\% & -2.23 & 5467.11 & 1551.15 & 19.08\% & -1.57 & 951.58 & 875.88 & 62.78\% & -1.28 & 1273.53 & 699.50 & 44.93\% & -2.13 & 375.88 & 67.67 & 81.87\% & -1.97 & 497.87 & 178.80 & 70.03\% & -2.12 \\ 
4g6m & -8.60 & -21.61 & 50.00\% & -2.64 & 6745.18 & 155.15 & 38.06\% & -2.00 & 5037.48 & 813.40 & 30.38\% & -2.01 & 2035.59 & 1358.96 & 47.35\% & -2.25 & 848.30 & 664.43 & 40.19\% & -2.04 & 280.47 & 88.75 & 66.93\% & -2.05 & 350.47 & 297.03 & 47.83\% & -1.96 \\ 
4h8w & -1.33 & -12.71 & 50.00\% & -1.84 & 12369.63 & 249.56 & 41.41\% & -2.05 & 7265.88 & 491.25 & 19.01\% & -1.72 & 3124.85 & 1281.34 & 30.86\% & -1.51 & 1297.18 & 672.89 & 48.22\% & -2.01 & 618.75 & 171.74 & 60.98\% & -2.06 & 1107.27 & 264.67 & 42.45\% & -2.00 \\ 
4ki5 & -8.15 & -16.58 & 26.67\% & -1.80 & 4689.92 & 667.19 & 37.81\% & -1.93 & 8141.08 & 69.59 & 39.48\% & -1.51 & 4663.15 & -0.12 & 33.85\% & -2.28 & 2494.06 & 2181.34 & 36.35\% & -2.12 & 776.62 & 429.83 & 68.58\% & -2.42 & 1646.62 & 893.89 & 35.31\% & -2.20 \\ 
4lvn & 40.37 & -11.59 & 46.15\% & -3.05 & 7876.98 & 178.24 & 40.79\% & -1.98 & 6142.84 & 120.48 & 39.66\% & -1.68 & 3396.91 & 103.42 & 53.89\% & -1.37 & 3260.43 & 511.25 & 46.31\% & -2.12 & 1042.90 & 19.44 & 73.28\% & -2.20 & 1831.02 & 357.13 & 47.60\% & -1.97 \\ 
4ot1 & -11.19 & -25.77 & 41.67\% & -2.50 & 9108.96 & 1197.97 & 38.04\% & -2.19 & 26107.87 & 2167.05 & 63.56\% & -2.20 & 18833.98 & 5614.24 & 39.15\% & -1.52 & 3532.15 & 3014.32 & 32.81\% & -2.16 & 1384.44 & 1122.83 & 70.01\% & -2.27 & 1972.81 & 1404.79 & 38.15\% & -2.00 \\ 
4qci & 14.31 & -3.35 & 53.85\% & -2.61 & 2648.94 & 841.19 & 39.06\% & -2.09 & 5365.28 & 0.06 & 28.97\% & -1.63 & 2043.48 & 48.25 & 24.64\% & -1.80 & 537.96 & 0.39 & 40.56\% & -2.10 & 129.25 & -0.12 & 62.42\% & -2.28 & 170.91 & 0.63 & 44.31\% & -2.15 \\ 
4xnq & -18.37 & -20.88 & 75.00\% & -1.89 & 14375.34 & 1055.40 & 40.14\% & -2.06 & 9305.46 & 586.48 & 27.67\% & -2.19 & 6710.95 & 215.05 & 24.45\% & -1.97 & 1601.98 & 541.82 & 34.51\% & -2.22 & 582.21 & 125.31 & 74.48\% & -2.64 & 1239.99 & 274.35 & 34.38\% & -2.25 \\ 
4ydk & -30.59 & -35.64 & 36.36\% & -2.55 & 20568.19 & 203.12 & 38.42\% & -2.27 & 25670.41 & 1852.50 & 27.23\% & -2.33 & 10877.30 & 2840.50 & 40.41\% & -1.81 & 4397.02 & 2551.16 & 31.37\% & -2.24 & 1738.58 & 875.15 & 63.92\% & -2.31 & 2721.85 & 1232.94 & 33.43\% & -2.18 \\ 
5b8c & -4.19 & -15.23 & 38.46\% & -1.80 & 5093.61 & 967.04 & 40.42\% & -1.45 & 6173.73 & 1110.47 & 29.13\% & -1.50 & 4293.39 & 261.41 & 30.77\% & -1.66 & 968.21 & 658.75 & 44.87\% & -1.62 & 178.36 & 19.48 & 77.04\% & -2.28 & 551.45 & 255.05 & 52.84\% & -1.70 \\ 
5bv7 & 44.87 & -18.25 & 47.37\% & -1.73 & 11453.29 & 1659.55 & 38.62\% & -1.88 & 16485.45 & 382.40 & 56.09\% & -2.12 & 4103.66 & 142.34 & 47.29\% & -2.29 & 2561.50 & 2520.19 & 36.27\% & -1.73 & 1389.85 & 1377.79 & 61.02\% & -2.00 & 1727.75 & 1862.98 & 37.53\% & -1.58 \\ 
5d93 & -6.28 & -6.83 & 44.44\% & -2.28 & 9596.77 & 229.00 & 43.81\% & -2.01 & 2602.18 & 655.98 & 24.07\% & -1.75 & 304.67 & 89.91 & 46.99\% & -1.77 & 838.21 & 268.25 & 48.78\% & -2.10 & 313.05 & 66.16 & 62.85\% & -1.99 & 483.98 & 184.26 & 35.24\% & -1.81 \\ 
5en2 & -20.91 & -8.44 & 35.29\% & -1.95 & 13321.21 & 2276.21 & 39.46\% & -2.04 & 9855.49 & 936.62 & 33.15\% & -1.85 & 4739.77 & 994.38 & 32.41\% & -2.02 & 2665.76 & 1961.80 & 26.65\% & -2.13 & 436.19 & 160.37 & 74.27\% & -2.15 & 1236.57 & 734.00 & 38.51\% & -1.95 \\ 
5f9o & 5.96 & -16.16 & 46.67\% & -2.71 & 6967.16 & 741.87 & 37.67\% & -2.06 & 6681.43 & 1733.31 & 29.48\% & -1.99 & 5657.30 & 33.28 & 27.19\% & -2.32 & 2028.59 & 1955.59 & 41.70\% & -2.16 & 362.41 & 40.84 & 82.55\% & -2.43 & 1083.65 & 431.15 & 46.08\% & -2.07 \\ 
5ggs & -15.18 & -17.75 & 38.46\% & -2.51 & 7470.50 & 731.35 & 38.54\% & -2.03 & 6708.07 & 992.69 & 28.21\% & -1.47 & 4005.27 & 1021.12 & 30.77\% & -1.68 & 1175.68 & 834.52 & 43.79\% & -2.11 & 205.83 & 10.38 & 89.51\% & -2.17 & 480.12 & 235.27 & 58.93\% & -2.04 \\ 
5hi4 & 0.48 & -18.07 & 45.45\% & -2.34 & 11977.15 & 17652.16 & 42.90\% & -2.25 & 5135.00 & 1710.83 & 18.84\% & -1.50 & 1138.60 & 1116.42 & 54.55\% & -1.64 & 1472.07 & 1053.91 & 46.73\% & -2.27 & 460.46 & 100.91 & 64.11\% & -2.05 & 854.79 & 346.15 & 42.00\% & -2.06 \\ 
5j13 & 0.61 & -18.76 & 60.00\% & -2.06 & 12601.91 & 3531.94 & 37.15\% & -1.90 & 6211.06 & 547.59 & 34.72\% & -1.99 & 7589.29 & 6606.01 & 34.83\% & -2.39 & 1821.92 & 2245.62 & 44.97\% & -2.21 & 384.44 & 66.18 & 86.01\% & -2.03 & 760.26 & 219.79 & 63.78\% & -2.08 \\ 
5l6y & -0.45 & -10.43 & 46.67\% & -1.94 & 17597.70 & 609.49 & 35.69\% & -1.96 & 7367.48 & 349.13 & 17.22\% & -1.91 & 4201.51 & 1432.54 & 32.36\% & -2.31 & 1322.21 & 384.84 & 45.79\% & -2.14 & 557.41 & 26.68 & 66.15\% & -2.18 & 920.33 & 79.18 & 42.33\% & -1.98 \\ 
5mes & -16.95 & -7.42 & 66.67\% & -2.39 & 9098.84 & 391.62 & 41.23\% & -2.14 & 5031.27 & 89.94 & 31.51\% & -1.32 & 1979.26 & 1613.61 & 33.72\% & -2.45 & 766.11 & 359.95 & 47.44\% & -2.17 & 185.66 & 62.14 & 71.14\% & -2.19 & 323.58 & 86.86 & 50.61\% & -2.07 \\ 
5nuz & -16.73 & -18.19 & 23.08\% & -2.16 & 13795.67 & 641.68 & 40.83\% & -1.99 & 6690.16 & 1012.48 & 25.64\% & -2.17 & 1746.62 & 368.08 & 38.66\% & -2.15 & 2199.90 & 2384.32 & 33.21\% & -2.14 & 1247.62 & 1057.81 & 54.85\% & -2.03 & 1649.31 & 1431.98 & 37.70\% & -2.02 \\

\bottomrule
\end{longtable}

% \renewcommand{\arraystretch}{1}
}







% \begin{longtable}{c|c|c}
%     \hline
%     Header 1 & Header 2 & Header 3 \\
%     \hline
%     \endfirsthead
%     \multicolumn{3}{|c|}%
%     {Table continues} \\
%         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\ 
%     \endhead
%     \hline
%             Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\ 
%             Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\ 
%     \multicolumn{3}{|r|}{Continued on next page} \\ \hline
%     \endfoot
%     Entry 1 & Entry 2 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\ 
%     ... & ... & ... \\ 
% \end{longtable}

==> tables/all_complexes_revision_top1.tex <==
{\tiny
% Reduce the font size
\setlength{\tabcolsep}{2pt} % Reduce the column separation
% \renewcommand{\arraystretch}{1.2}
\begin{longtable}{c|rrrr|rrrr|rrrr|rrrr|rrrr|rrrr|rrrr}
\caption{Detailed evaluation results for reference antibodies and top-1 antibodies designed by HERN, MEAN, dyMEAN, DiffAb, \method, and \methodp for 55 antigens. The data source is the same as that in \cref{tab:top_1}. For simplicity, we use A, B, C, and D to stand for CDR $E_{\text{total}}$, CDR-Ag $\Delta G$, PHR, and pLL respectively in this table. The unit of the two energies is kcal/mol and omitted for brevity.}\label{tab:all_complexes_top1}
\endfirsthead
\endhead
\toprule
% \diagbox{Model}{Metric} 


\multirow{2}{*}{\textbf{PDB id}} 
& \multicolumn{4}{c|}{\textbf{RAbD (Reference)}}
& \multicolumn{4}{c|}{\textbf{HERN}}
 & \multicolumn{4}{c|}{\textbf{MEAN}}
  & \multicolumn{4}{c|}{\textbf{dyMEAN}}
  & \multicolumn{4}{c|}{\textbf{DiffAb}}
    & \multicolumn{4}{c|}{\textbf{\method}}
        & \multicolumn{4}{c}{\textbf{\methodp}}
\\
& A&B&C&D& A&B&C&D& A&B&C&D& A&B&C&D& A&B&C&D & A&B&C&D& A&B&C&D\\
\midrule
1a14 & 62.28 & -4.72 & 40.00\% & -1.56 & 3370.02 & -1.79 & 26.67\% & -1.01 & 5142.76 & -2.97 & 26.67\% & -1.81 & 3521.78 & -2.04 & 46.67\% & -1.80 & 298.23 & -6.50 & 20.00\% & -1.97 & \textcolor{red}{\textbf{44.65}} & \textcolor{red}{\textbf{-5.83}} & 86.67\% & -2.25 & 189.19 & 1.23 & 26.67\% & -1.02 \\ 
1a2y & -22.18 & -4.81 & 20.00\% & -1.30 & 6101.92 & -1.35 & 50.00\% & -1.46 & 2259.30 & -1.43 & 40.00\% & -0.84 & 61.49 & -0.06 & 60.00\% & -1.15 & 125.47 & -1.84 & 40.00\% & -1.12 & 20.87 & -3.58 & 60.00\% & -2.43 & 74.95 & -5.61 & 20.00\% & -1.35 \\ 
1fe8 & 25.79 & -14.84 & 44.44\% & -2.61 & 3663.52 & -1.34 & 55.56\% & -2.16 & 1721.37 & 3.69 & 44.44\% & -1.69 & 823.80 & 221.87 & 55.56\% & -1.93 & 332.67 & 14.57 & 44.44\% & -2.03 & 127.38 & -8.11 & 33.33\% & -2.49 & 667.06 & -6.12 & 22.22\% & -1.75 \\ 
1ic7 & 19.96 & -2.62 & 57.14\% & -2.89 & 4871.00 & -2.07 & 42.86\% & -1.69 & 525.84 & -2.26 & 28.57\% & -2.03 & 413.21 & 60.26 & 42.86\% & -1.45 & 131.09 & -1.73 & 42.86\% & -2.15 & \textcolor{red}{\textbf{-1.63}} & \textcolor{red}{\textbf{-3.50}} & 71.43\% & -1.43 & \textcolor{red}{\textbf{8.08}} & \textcolor{red}{\textbf{-3.57}} & 42.86\% & -0.89 \\ 
1iqd & 43.36 & -5.47 & 70.00\% & -2.66 & 8950.62 & -0.63 & 50.00\% & -1.99 & 1343.07 & -3.17 & 70.00\% & -3.13 & 502.21 & -1.48 & 60.00\% & -1.97 & 229.08 & -1.67 & 50.00\% & -2.06 & \textcolor{red}{\textbf{12.71}} & \textcolor{red}{\textbf{-7.36}} & 90.00\% & -2.22 & 131.10 & 47.91 & 50.00\% & -1.81 \\ 
1n8z & 41.88 & -8.00 & 53.85\% & -2.50 & 5547.03 & 6.55 & 46.15\% & -2.08 & 2886.71 & 5.78 & 23.08\% & -2.34 & 1804.53 & -2.52 & 53.85\% & -2.05 & 326.22 & -0.53 & 38.46\% & -2.18 & 106.81 & -3.20 & 38.46\% & -2.38 & 101.78 & 40.02 & 30.77\% & -1.51 \\ 
1ncb & 29.72 & -11.94 & 38.46\% & -2.35 & 13605.15 & 357.59 & 46.15\% & -1.95 & 4130.61 & 624.22 & 23.08\% & -1.27 & 6597.50 & 4301.46 & 30.77\% & -2.15 & 631.94 & 150.24 & 53.85\% & -2.25 & 159.57 & -6.33 & 76.92\% & -2.19 & 1095.23 & 2.21 & 30.77\% & -1.81 \\ 
1osp & -1.39 & -15.94 & 42.86\% & -1.78 & 17731.35 & 32650.25 & 57.14\% & -1.74 & 2693.69 & 34.23 & 57.14\% & -1.88 & 8881.64 & 12416.92 & 50.00\% & -1.76 & 237.19 & 9.82 & 57.14\% & -2.49 & 59.01 & -5.55 & 78.57\% & -2.18 & 184.27 & -4.81 & 28.57\% & -1.37 \\ 
1uj3 & -12.93 & -11.45 & 40.00\% & -2.16 & 11290.58 & -0.51 & 40.00\% & -2.05 & 1709.16 & -2.04 & 50.00\% & -1.38 & 660.71 & 36.96 & 60.00\% & -1.68 & 264.93 & 16.69 & 40.00\% & -2.28 & 34.84 & -5.71 & 60.00\% & -2.42 & 216.60 & 0.72 & 20.00\% & -1.91 \\ 
1w72 & 8.36 & -16.06 & 46.67\% & -2.05 & 10076.18 & 88.75 & 40.00\% & -1.92 & 4196.89 & 0.74 & 26.67\% & -1.49 & 4162.03 & 1206.78 & 33.33\% & -2.34 & 386.12 & 4.72 & 66.67\% & -1.95 & 119.22 & -1.51 & 80.00\% & -1.88 & 739.00 & 165.90 & 33.33\% & -1.27 \\ 
2adf & -20.47 & -15.53 & 36.36\% & -2.16 & 8781.28 & -2.78 & 45.45\% & -2.16 & 2996.23 & 361.67 & 27.27\% & -1.89 & 788.08 & 81.23 & 54.55\% & -2.05 & 174.54 & 9.10 & 63.64\% & -2.11 & 82.61 & -7.50 & 63.64\% & -2.29 & 787.24 & 6.15 & 27.27\% & -1.87 \\ 
2b2x & 5.41 & -0.90 & 58.33\% & -2.22 & 7922.20 & -1.74 & 50.00\% & -2.44 & 7299.02 & -3.12 & 25.00\% & -1.54 & 2916.38 & 2284.43 & 41.67\% & -1.07 & 479.11 & -1.18 & 66.67\% & -2.09 & 83.46 & -4.01 & 66.67\% & -2.26 & 257.80 & -3.84 & 41.67\% & -1.57 \\ 
2cmr & 5.25 & -9.79 & 41.67\% & -2.20 & 13987.00 & 88.57 & 50.00\% & -2.00 & 3548.46 & 201.80 & 33.33\% & -1.18 & 3024.63 & 869.16 & 50.00\% & -1.78 & 341.10 & 17.00 & 66.67\% & -2.53 & 134.20 & -4.00 & 50.00\% & -1.74 & 502.95 & 16.40 & 33.33\% & -1.62 \\ 
2dd8 & 68.27 & -7.21 & 63.64\% & -2.27 & 8801.59 & 131.33 & 72.73\% & -2.43 & 4785.61 & -5.17 & 18.18\% & -1.59 & 1814.99 & 960.05 & 54.55\% & -1.54 & 214.55 & -4.85 & 36.36\% & -2.25 & \textcolor{red}{\textbf{28.07}} & \textcolor{red}{\textbf{-8.74}} & 63.64\% & -2.21 & 343.40 & -4.26 & 36.36\% & -1.62 \\ 
2vxt & -10.32 & -12.95 & 66.67\% & -1.76 & 4792.96 & -0.78 & 66.67\% & -2.53 & 645.86 & 14.70 & 16.67\% & -1.72 & 191.22 & 117.11 & 50.00\% & -1.11 & 48.87 & -2.00 & 66.67\% & -1.61 & 2.26 & -6.55 & 83.33\% & -2.11 & 16.92 & -4.38 & 50.00\% & -1.35 \\ 
2xqy & -3.67 & -16.14 & 54.55\% & -2.68 & 9737.32 & -0.83 & 36.36\% & -1.94 & 1266.63 & -0.72 & 63.64\% & -1.63 & 1528.26 & 550.52 & 45.45\% & -0.76 & 222.91 & -1.87 & 36.36\% & -2.40 & 23.11 & -7.45 & 63.64\% & -2.09 & 63.48 & -3.19 & 36.36\% & -1.15 \\ 
2xwt & -19.96 & -27.99 & 50.00\% & -2.57 & 11584.12 & -0.06 & 50.00\% & -2.14 & 4082.86 & 104.45 & 16.67\% & -1.94 & 3180.46 & 2638.26 & 33.33\% & -2.36 & 485.02 & 4.74 & 41.67\% & -1.87 & 35.10 & -4.60 & 66.67\% & -1.94 & 349.68 & -1.46 & 33.33\% & -1.64 \\ 
2ypv & 4.72 & -6.94 & 25.00\% & -1.43 & 15216.10 & 86.25 & 50.00\% & -1.77 & 3475.66 & 1053.53 & 33.33\% & -1.41 & 4417.05 & 6151.36 & 25.00\% & -1.10 & 621.23 & 295.98 & 41.67\% & -1.94 & 65.47 & -2.90 & 66.67\% & -2.28 & 227.20 & 119.80 & 33.33\% & -1.63 \\ 
3bn9 & 81.92 & -0.89 & 33.33\% & -1.71 & 11004.75 & 0.37 & 55.56\% & -2.06 & 3153.02 & -2.19 & 44.44\% & -1.94 & 7742.77 & -0.36 & 66.67\% & -1.91 & 573.75 & -2.38 & 55.56\% & -2.04 & \textcolor{red}{\textbf{59.96}} & \textcolor{red}{\textbf{-3.11}} & 55.56\% & -2.73 & 362.72 & -1.73 & 22.22\% & -1.49 \\ 
3cx5 & -18.25 & -14.91 & 33.33\% & -1.80 & 14437.58 & 462.31 & 40.00\% & -1.67 & 4322.29 & -5.07 & 46.67\% & -1.22 & 4842.11 & 45.60 & 40.00\% & -1.37 & 134.10 & -4.86 & 46.67\% & -1.61 & 35.44 & -10.11 & 60.00\% & -1.36 & 405.94 & -5.34 & 26.67\% & -1.07 \\ 
3ffd & 43.13 & -12.63 & 36.36\% & -2.39 & 2076.23 & -3.98 & 45.45\% & -2.24 & 1419.27 & 1.47 & 54.55\% & -1.75 & 502.53 & 615.53 & 54.55\% & -1.76 & 125.43 & 164.91 & 45.45\% & -1.98 & 40.23 & -1.87 & 45.45\% & -2.32 & 175.01 & 81.20 & 18.18\% & -1.79 \\ 
3hi6 & -1.47 & -12.35 & 46.15\% & -1.93 & 11018.30 & -6.46 & 53.85\% & -1.92 & 6648.87 & 2889.20 & 23.08\% & -1.88 & 2511.50 & 1888.22 & 61.54\% & -2.20 & 536.27 & 243.63 & 61.54\% & -2.07 & 149.54 & -5.65 & 84.62\% & -1.87 & 388.65 & 81.17 & 38.46\% & -1.73 \\ 
3k2u & 18.71 & -14.57 & 72.73\% & -3.02 & 8174.07 & -1.96 & 54.55\% & -2.23 & 3213.40 & 1028.78 & 36.36\% & -1.00 & 886.48 & 1171.60 & 54.55\% & -1.33 & 136.63 & 35.80 & 45.45\% & -1.74 & 18.86 & -3.10 & 63.64\% & -2.10 & 201.56 & 8.50 & 27.27\% & -1.62 \\ 
3l95 & -1.18 & -18.48 & 58.33\% & -2.50 & 13351.29 & -1.70 & 41.67\% & -2.15 & 4472.76 & 115.65 & 33.33\% & -1.98 & 968.84 & 276.55 & 66.67\% & -1.49 & 312.03 & 1.23 & 41.67\% & -1.70 & 73.09 & -7.27 & 58.33\% & -1.56 & 206.67 & -1.48 & 33.33\% & -1.35 \\ 
3mxw & -7.55 & -19.04 & 41.67\% & -2.10 & 6712.93 & 7.23 & 33.33\% & -1.92 & 3141.84 & 4.10 & 33.33\% & -2.27 & 3247.51 & 1354.59 & 33.33\% & -1.90 & 172.90 & 4.59 & 66.67\% & -2.00 & 29.67 & -4.00 & 83.33\% & -2.39 & 94.21 & -2.64 & 41.67\% & -1.61 \\ 
3nid & -21.55 & -28.54 & 41.67\% & -2.06 & 8480.65 & 123.17 & 50.00\% & -2.22 & 6265.25 & 1813.79 & 25.00\% & -1.69 & 685.91 & 626.38 & 58.33\% & -1.82 & 540.87 & 407.11 & 50.00\% & -1.92 & 59.61 & -4.63 & 75.00\% & -2.56 & 926.30 & 467.72 & 25.00\% & -1.85 \\ 
3o2d & 0.23 & -13.42 & 46.67\% & -2.01 & 4273.90 & 735.38 & 53.33\% & -1.77 & 4629.39 & -1.23 & 40.00\% & -1.44 & 2530.49 & -0.98 & 46.67\% & -1.53 & 388.39 & 0.90 & 26.67\% & -2.40 & 49.28 & -3.62 & 93.33\% & -2.33 & 235.27 & -1.20 & 40.00\% & -1.28 \\ 
3rkd & -6.61 & -10.35 & 43.75\% & -1.94 & 1818.15 & 124.59 & 37.50\% & -2.07 & 4126.58 & -4.75 & 56.25\% & -2.10 & 1748.64 & 6.24 & 37.50\% & -2.18 & 576.71 & 7.22 & 43.75\% & -2.00 & 77.66 & -5.85 & 75.00\% & -2.71 & 337.99 & -3.64 & 25.00\% & -1.68 \\ 
3s35 & -4.63 & -5.60 & 20.00\% & -2.23 & 6506.10 & 7.92 & 60.00\% & -2.22 & 1638.19 & 99.18 & 30.00\% & -0.95 & 919.12 & 962.83 & 60.00\% & -1.44 & 75.14 & 22.60 & 60.00\% & -1.67 & 11.55 & -7.60 & 80.00\% & -2.16 & 36.60 & -4.65 & 60.00\% & -1.69 \\ 
3w9e & -9.93 & -18.41 & 40.00\% & -2.29 & 14363.44 & 799.14 & 46.67\% & -1.98 & 4551.50 & 518.30 & 33.33\% & -1.65 & 8590.08 & 11529.24 & 40.00\% & -2.17 & 545.30 & 26.61 & 33.33\% & -1.76 & 103.21 & -5.46 & 73.33\% & -1.94 & 555.46 & 3.26 & 33.33\% & -1.08 \\ 
4cmh & -19.18 & -16.54 & 30.77\% & -1.63 & 7821.21 & 60.38 & 46.15\% & -1.81 & 6314.53 & 424.01 & 38.46\% & -1.26 & 4680.21 & 1388.22 & 30.77\% & -1.95 & 710.43 & 774.04 & 53.85\% & -1.97 & 50.34 & 1.41 & 84.62\% & -1.89 & 671.25 & 145.64 & 46.15\% & -1.34 \\ 
4dtg & 7.56 & -5.43 & 50.00\% & -2.31 & 9843.25 & 16234.71 & 50.00\% & -2.01 & 1817.18 & -0.84 & 57.14\% & -1.67 & 1259.81 & 73.30 & 50.00\% & -1.84 & 77.78 & 20.77 & 35.71\% & -2.12 & 41.75 & -4.41 & 85.71\% & -2.06 & 127.02 & 3.63 & 35.71\% & -1.76 \\ 
4dvr & -6.74 & 1.13 & 66.67\% & -2.89 & 8851.78 & -2.11 & 50.00\% & -2.01 & 2228.20 & -1.62 & 41.67\% & -1.21 & 2315.58 & 790.43 & 33.33\% & -2.57 & 189.44 & -2.10 & 50.00\% & -1.95 & 13.89 & -5.43 & 75.00\% & -2.51 & 70.08 & -1.22 & 33.33\% & -1.84 \\ 
4ffv & 28.69 & 0.67 & 50.00\% & -2.96 & 1142.48 & -0.89 & 50.00\% & -2.25 & 1265.17 & -4.00 & 20.00\% & -1.63 & 425.73 & -0.51 & 70.00\% & -1.48 & 151.06 & -1.29 & 50.00\% & -1.71 & 44.35 & -2.34 & 60.00\% & -2.19 & 96.61 & -3.81 & 50.00\% & -1.51 \\ 
4fqj & 33.50 & -21.93 & 38.89\% & -1.66 & 12660.96 & 48.19 & 44.44\% & -1.94 & 4163.98 & 87.78 & 38.89\% & -2.34 & 5274.34 & 531.42 & 44.44\% & -2.14 & 966.00 & 475.91 & 38.89\% & -1.81 & 151.09 & 1.40 & 77.78\% & -2.13 & 869.39 & 267.80 & 16.67\% & -1.68 \\ 
4g6j & 0.30 & -8.81 & 45.45\% & -1.92 & 8685.25 & 34.14 & 45.45\% & -2.13 & 3910.08 & 189.16 & 18.18\% & -2.57 & 796.48 & 628.64 & 63.64\% & -1.29 & 212.73 & 0.48 & 63.64\% & -2.02 & 31.88 & -3.53 & 81.82\% & -2.03 & 72.92 & -3.63 & 54.55\% & -1.62 \\ 
4g6m & -8.60 & -21.61 & 50.00\% & -2.64 & 5173.21 & -0.57 & 41.67\% & -2.04 & 2615.09 & 74.92 & 41.67\% & -1.76 & 1650.47 & 1053.70 & 50.00\% & -2.09 & 14.30 & -1.55 & 41.67\% & -2.01 & 11.82 & -5.27 & 66.67\% & -2.16 & 20.32 & -5.38 & 33.33\% & -1.87 \\ 
4h8w & -1.33 & -12.71 & 50.00\% & -1.84 & 10178.09 & -1.14 & 66.67\% & -2.09 & 4219.10 & -0.12 & 16.67\% & -1.65 & 1347.02 & 266.59 & 41.67\% & -2.18 & 407.69 & 5.12 & 50.00\% & -2.04 & 53.51 & -5.07 & 75.00\% & -1.90 & 312.93 & -3.84 & 25.00\% & -1.66 \\ 
4ki5 & -8.15 & -16.58 & 26.67\% & -1.80 & 2626.19 & 27.58 & 46.67\% & -1.93 & 4943.25 & -0.55 & 40.00\% & -1.44 & 3439.33 & -1.96 & 40.00\% & -1.90 & 1027.67 & 3.06 & 40.00\% & -1.79 & 74.95 & -5.23 & 73.33\% & -2.36 & 318.38 & -0.54 & 33.33\% & -1.72 \\ 
4lvn & 40.37 & -11.59 & 46.15\% & -3.05 & 5298.71 & 95.21 & 53.85\% & -1.80 & 2298.31 & -2.59 & 38.46\% & -1.67 & 1920.97 & 25.46 & 61.54\% & -1.63 & 1481.29 & -5.19 & 69.23\% & -2.36 & 254.52 & -4.81 & 76.92\% & -2.17 & 1362.36 & -4.38 & 30.77\% & -1.40 \\ 
4ot1 & -11.19 & -25.77 & 41.67\% & -2.50 & 5396.84 & 372.36 & 41.67\% & -2.13 & 14659.75 & 500.72 & 66.67\% & -2.18 & 14443.68 & 4020.89 & 41.67\% & -1.13 & 1069.16 & -1.03 & 41.67\% & -2.03 & 242.35 & -4.61 & 50.00\% & -1.71 & 492.04 & 161.16 & 25.00\% & -1.66 \\ 
4qci & 14.31 & -3.35 & 53.85\% & -2.61 & 1380.37 & 130.53 & 38.46\% & -2.28 & 2667.14 & -0.28 & 38.46\% & -2.14 & 1599.80 & -0.38 & 23.08\% & -1.69 & 47.93 & -2.00 & 38.46\% & -2.04 & 20.01 & -2.29 & 53.85\% & -2.23 & 39.84 & -3.76 & 30.77\% & -1.71 \\ 
4xnq & -18.37 & -20.88 & 75.00\% & -1.89 & 10639.18 & 73.24 & 56.25\% & -2.24 & 5229.34 & 61.78 & 37.50\% & -2.31 & 5711.22 & 123.66 & 25.00\% & -1.93 & 714.34 & -0.51 & 43.75\% & -2.33 & 70.23 & -4.44 & 68.75\% & -2.60 & 311.06 & 3.14 & 18.75\% & -1.64 \\ 
4ydk & -30.59 & -35.64 & 36.36\% & -2.55 & 14084.25 & -0.35 & 31.82\% & -2.40 & 14107.70 & 17.93 & 31.82\% & -2.47 & 8232.12 & 1800.22 & 40.91\% & -1.40 & 1586.95 & 171.24 & 50.00\% & -2.26 & 121.44 & -6.48 & 68.18\% & -2.23 & 938.56 & 28.09 & 22.73\% & -2.00 \\ 
5b8c & -4.19 & -15.23 & 38.46\% & -1.80 & 3575.88 & 34.60 & 46.15\% & -1.57 & 3630.36 & -4.90 & 38.46\% & -1.39 & 3476.96 & 141.64 & 30.77\% & -1.66 & 171.90 & -1.86 & 61.54\% & -1.70 & 40.35 & -6.90 & 76.92\% & -1.63 & 312.28 & -6.37 & 38.46\% & -0.87 \\ 
5bv7 & 44.87 & -18.25 & 47.37\% & -1.73 & 8940.31 & 428.40 & 36.84\% & -1.44 & 7124.46 & 8.81 & 57.89\% & -1.82 & 3557.20 & 81.48 & 47.37\% & -2.30 & 502.22 & 10.37 & 36.84\% & -2.10 & 88.84 & -7.49 & 73.68\% & -2.04 & 381.55 & 28.72 & 21.05\% & -1.25 \\ 
5d93 & -6.28 & -6.83 & 44.44\% & -2.28 & 7994.29 & 198.09 & 44.44\% & -2.00 & 1327.34 & -2.50 & 44.44\% & -1.60 & 91.41 & -2.97 & 55.56\% & -1.89 & 70.24 & -3.18 & 55.56\% & -2.07 & 18.64 & -4.53 & 66.67\% & -2.12 & 91.64 & -4.49 & 33.33\% & -1.36 \\ 
5en2 & -20.91 & -8.44 & 35.29\% & -1.95 & 10072.38 & 1401.50 & 47.06\% & -1.71 & 5079.34 & 25.09 & 35.29\% & -1.65 & 3919.12 & 26.12 & 41.18\% & -1.76 & 521.48 & 83.93 & 35.29\% & -2.19 & 118.27 & -6.66 & 64.71\% & -2.11 & 404.68 & 53.20 & 23.53\% & -1.66 \\ 
5f9o & 5.96 & -16.16 & 46.67\% & -2.71 & 5406.24 & 413.41 & 33.33\% & -2.03 & 3770.48 & 622.27 & 40.00\% & -1.45 & 4852.12 & -1.04 & 33.33\% & -2.21 & 345.58 & 147.83 & 53.33\% & -2.27 & 85.64 & -3.61 & 86.67\% & -2.40 & 184.90 & -3.97 & 26.67\% & -1.99 \\ 
5ggs & -15.18 & -17.75 & 38.46\% & -2.51 & 5621.88 & 36.53 & 46.15\% & -2.14 & 4429.14 & 124.02 & 23.08\% & -1.78 & 3285.12 & 930.05 & 30.77\% & -1.68 & 206.95 & -3.74 & 61.54\% & -2.22 & 34.25 & -8.49 & 92.31\% & -2.18 & 138.10 & -9.29 & 46.15\% & -1.55 \\ 
5hi4 & 0.48 & -18.07 & 45.45\% & -2.34 & 9789.87 & 13849.60 & 54.55\% & -2.21 & 3004.20 & 402.13 & 18.18\% & -1.57 & 991.65 & 588.91 & 54.55\% & -1.64 & 186.35 & 0.53 & 54.55\% & -1.86 & 89.25 & -5.44 & 72.73\% & -1.83 & 377.22 & -3.98 & 27.27\% & -1.13 \\ 
5j13 & 0.61 & -18.76 & 60.00\% & -2.06 & 8911.86 & 2045.54 & 73.33\% & -1.86 & 2597.89 & -0.96 & 53.33\% & -1.91 & 4840.53 & 4973.45 & 46.67\% & -2.41 & 135.69 & 0.30 & 66.67\% & -2.27 & 55.16 & -6.97 & 66.67\% & -2.39 & 124.44 & -1.07 & 46.67\% & -1.79 \\ 
5l6y & -0.45 & -10.43 & 46.67\% & -1.94 & 15653.52 & 127.28 & 53.33\% & -2.21 & 2982.89 & -0.05 & 33.33\% & -1.82 & 2987.61 & 1163.43 & 33.33\% & -2.34 & 134.68 & -2.59 & 66.67\% & -2.14 & 55.10 & -3.54 & 66.67\% & -1.84 & 154.32 & -3.89 & 33.33\% & -1.62 \\ 
5mes & -16.95 & -7.42 & 66.67\% & -2.39 & 7281.40 & 45.85 & 50.00\% & -2.23 & 2132.88 & -2.61 & 41.67\% & -1.02 & 1377.29 & 1421.52 & 41.67\% & -2.29 & 186.88 & -2.91 & 58.33\% & -2.05 & 28.39 & -4.54 & 75.00\% & -2.31 & 211.29 & -3.27 & 33.33\% & -1.35 \\ 
5nuz & -16.73 & -18.19 & 23.08\% & -2.16 & 11978.97 & -1.37 & 53.85\% & -1.95 & 3901.04 & 80.63 & 38.46\% & -1.74 & 1394.59 & 230.11 & 46.15\% & -1.91 & 213.66 & 162.44 & 38.46\% & -2.39 & 126.07 & -4.80 & 61.54\% & -2.15 & 300.00 & -3.14 & 30.77\% & -1.51 \\ 

\bottomrule
\end{longtable}
% \renewcommand{\arraystretch}{1}
}


==> tables/full_average_metrics.tex <==
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
     \multirow{2}{*}{Method}
     & \multicolumn{2}{c|}{CDR $E_{\text{total}}$ ($\downarrow$)}
     % & CDR $E_{\text{total}}$ 
     & \multicolumn{2}{c|}{CDR-Ag $E_{\text{nonRep}}$}
     % & CDR-Ag $E_{\text{nonRep}}$
     & \multicolumn{2}{c|}{CDR-Ag $E_{\text{Rep}}$}
     % & CDR-Ag $E_{\text{Rep}}$
     & \multicolumn{2}{c}{CDR-Ag $\Delta G$ ($\downarrow$)}
     % & and CDR-Ag $\Delta G$
     % &  CDR\_avg &  CDR\_med & HsR\_nonRep\_avg & HsR\_nonRep\_med & HsR\_Rep\_avg & HsR\_Rep\_med & HsR\_avg & HsR\_med \\
     \\
     &  Avg. & Med. & Avg. & Med. &  Avg. & Med. & Avg. & Med.  \\
\midrule
         HERN & 10930.68 & 10776.79 & -10.9 &  -5.32 &  3656.77 &  569.61 & 2000.32 & 306.79 \\
         MEAN & 7138 & 6011.53 &  -9.34 &  -6.82 & 1903.32 &  907.69 &  1037.49 & 491.49 \\
       dyMEAN & 17302.98 &  8157.17 & -14.94 &  -7.46 & 5411.50 &  893.88 & 2961.39 & 484.09 \\
dyMEAN* &  4078.22 &  2238.42 & -16.20 & -10.73 & 4240.43 & 1415.49 & 2316.04 & 769.99 \\
       DiffAb &  1592.73 &  1340.42 &  -9.10 &  -7.33 & 2168.43 & 1212.86 & 1183.54 & 658.39 \\
        AbDPO &   989.59 &   634.34 &  -6.19 &  -4.61 &  513.53 &   32.93 &  276.25 &  12.95 \\
\bottomrule
\end{tabular}

==> tables/full_average_success_rate.tex <==
\begin{tabular}{c|cccccccccc}
\toprule
       Method &    95\% &    90\% &   85\% &   80\% &   75\% &   70\% &   65\% &   60\% &   55\% &   50\% \\
\midrule
  HERN &     0.00 &  0.00 & 0.00 & 0.00 & 0.00&  0.00 &  0.00 &  0.00 &  0.00 &  0.00 \\
  MEAN &  0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
dyMEAN &  \cellcolor[RGB]{210, 255, 210}0.95 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
dyMEAN* &  \cellcolor[RGB]{210, 255, 210}1.40 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
DiffAb &  \cellcolor[RGB]{210, 255, 210}2.28 & \cellcolor[RGB]{210, 255, 210}0.80 & \cellcolor[RGB]{210, 255, 210}0.34 & \cellcolor[RGB]{210, 255, 210}0.14 & \cellcolor[RGB]{210, 255, 210}0.04 & \cellcolor[RGB]{210, 255, 210}0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\
 AbDPO & \cellcolor[RGB]{210, 255, 210}13.05 & \cellcolor[RGB]{210, 255, 210}5.02 & \cellcolor[RGB]{210, 255, 210}2.36 & \cellcolor[RGB]{210, 255, 210}1.00 & \cellcolor[RGB]{210, 255, 210}0.41 & \cellcolor[RGB]{210, 255, 210}0.10 & \cellcolor[RGB]{210, 255, 210}0.02 & 0.00 & 0.00 & 0.00 \\
\bottomrule
\end{tabular}

==> tables/main_result.tex <==
%\resizebox{\linewidth}{!}{%
% \renewcommand{\arraystretch}{1.}
\begin{tabular}{lrrrrr}
\toprule
% \diagbox{Model}{Metric} 
\multirow{2}{*}{Methods} & \multicolumn{2}{r}{CDR $E_{\text{total}}$ ($\downarrow$)} & \multicolumn{2}{r}{CDR-Ag $\Delta G$ ($\downarrow$)}  & Success  \\
 & Avg. & Med. & Avg. & Med. & Rate ($\uparrow$) \\
\midrule
Reference & 4.52 	& -1.33 & -13.72 & -14.54 & 100\%  \\
\midrule
HERN      & 7594.94 & 7825.92 & 1159.34 & 4.12 &  0\% \\
MEAN      & 3113.70 & 2583.48 & 114.98 & -0.92 &  0\% \\
%dyMEAN    & 15025.67 & 7426.4 & 2391 & 213.77 &  0\% \\
dyMEAN   & 3234.30 & 1690.91 & 1619.24 & 177.08 &  0\% \\
% \midrule
DiffAb & 211.00 & 155.77 & 9.54 & -1.97 & 14.55\% \\
\method & \textbf{162.75} & \textbf{124.62} & \textbf{-4.85} & \textbf{-5.24} & \textbf{27.27\%} \\
\bottomrule
\end{tabular}
%}%
% \renewcommand{\arraystretch}{1}

==> tables/rosetta_opt_success_rate.tex <==
\begin{tabular}{c|c|cccccccccc}
\toprule
PDB ID & Method &    95\% &    90\% &    85\% &   80\% &   75\% &   70\% &   65\% &   60\% &   55\% &   50\% \\
\midrule
      \multirow{2}{*}{1ncb} &     DiffAb &  96.88 &  84.38 &  43.75 & 34.38 & 28.12 & 18.75 & 12.50 &  6.25 &  \cellcolor[RGB]{255, 210, 210}0.00 &  \cellcolor[RGB]{255, 210, 210}0.00 \\
        &      AbDPO & 100.00 & 100.00 &  90.32 & 83.87 & 80.65 & 58.06 & 29.03 & 16.13 &  9.68 &  3.23 \\
        \midrule
      \multirow{2}{*}{2xwt} &     DiffAb & 100.00 &  90.00 &  80.00 & 63.33 & 56.67 & 40.00 & 20.00 & 13.33 &  6.67 &  \cellcolor[RGB]{255, 210, 210}0.00 \\
        &      AbDPO & 100.00 & 100.00 &  96.88 & 96.88 & 84.38 & 65.62 & 40.62 & 18.75 &  9.38 &  6.25 \\
        \midrule
      \multirow{2}{*}{1iqd} &     DiffAb &  93.55 &  87.10 &  64.52 & 51.61 & 45.16 & 29.03 & 25.81 & 12.90 &  9.68 &  6.45 \\
        &      AbDPO & 100.00 & 100.00 & 100.00 & 96.88 & 93.75 & 71.88 & 56.25 & 31.25 & 18.75 & 12.50 \\
        \midrule
      \multirow{2}{*}{1a14} &     DiffAb & 100.00 & 100.00 & 100.00 & 81.25 & 71.88 & 59.38 & 31.25 & 15.62 &  9.38 &  3.12 \\
        &      AbDPO & 100.00 & 100.00 & 100.00 & 81.25 & 59.38 & 21.88 & 15.62 &  9.38 &  9.38 &  6.25 \\
        \midrule
      \multirow{2}{*}{5ggs} &     DiffAb & 100.00 &  86.67 &  60.00 & 53.33 & 36.67 & 16.67 & 10.00 &  3.33 &  \cellcolor[RGB]{255, 210, 210}0.00 &  \cellcolor[RGB]{255, 210, 210}0.00 \\
        &      AbDPO & 100.00 & 100.00 &  90.32 & 90.32 & 80.65 & 70.97 & 45.16 & 35.48 & 22.58 & 12.90 \\
        \midrule
      \multirow{2}{*}{4ki5} &     DiffAb & 100.00 & 100.00 &  93.33 & 90.00 & 73.33 & 56.67 & 40.00 & 23.33 & 16.67 & 10.00 \\
        &      AbDPO & 100.00 & 100.00 & 100.00 & 96.67 & 86.67 & 76.67 & 66.67 & 60.00 & 36.67 & 20.00 \\
        \midrule
      \multirow{2}{*}{4cmh} &     DiffAb &  86.67 &  60.00 &  33.33 & 16.67 & 13.33 & 10.00 &  6.67 &  3.33 &  \cellcolor[RGB]{255, 210, 210}0.00 &  \cellcolor[RGB]{255, 210, 210}0.00 \\
        &      AbDPO & 100.00 &  96.77 &  90.32 & 83.87 & 74.19 & 67.74 & 54.84 & 41.94 & 38.71 & 22.58 \\
        \midrule
      \multirow{2}{*}{3hi6} &     DiffAb & 100.00 &  90.00 &  66.67 & 56.67 & 40.00 & 20.00 & 13.33 &  6.67 &  3.33 &  \cellcolor[RGB]{255, 210, 210}0.00 \\
        &      AbDPO & 100.00 &  96.88 &  96.88 & 93.75 & 87.50 & 75.00 & 53.12 & 43.75 & 37.50 & 18.75 \\
\bottomrule
\end{tabular}

==> tables/rosetta_optimization_results.tex <==
\begin{tabular}{c|cc|cc|c|cc|cc|c}
\toprule
% \diagbox{Model}{Metric} 
\multirow{3}{*}{PDB ID} & \multicolumn{5}{c|}{DiffAb + Rosseta Structure Optimization} & \multicolumn{5}{c}{\method + Rosseta Structure Optimization} \\
\cmidrule{2-11}
& \multicolumn{2}{c|}{CDR $E_{\text{total}}$ ($\downarrow$)} & \multicolumn{2}{c|}{CDR-Ag $\Delta G$ ($\downarrow$)}  & Success & \multicolumn{2}{c|}{CDR $E_{\text{total}}$ ($\downarrow$)} & \multicolumn{2}{c|}{CDR-Ag $\Delta G$ ($\downarrow$)}  & Success \\
 & Avg. & Med. & Avg. & Med. & Rate ($\uparrow$) & Avg. & Med. & Avg. & Med. & Rate ($\uparrow$)  \\
\midrule
1ncb  &  61.59 	& 59.04 & -0.00 & 0.19 &  0\%
    &   26.29 & 18.86 & -5.62 & -5.36 &  3.23\% \\
2xwt  & 41.84 & 35.25 & -3.38 & -2.97 & 0\%
    &   15.81 & 13.64 & -4.99 & -5.21 & 6.25\%
\\
1iqd  & 54.84 & 36.16 & -2.34 & -2.96 & 6.45\% 
    &  9.78 & 1.84 & -6.00 & -6.20 & 12.5\%
\\
% 1a14 & 20.50 & 15.14 & -4.38 & -4.70 & 
1a14   & 19.32 & 16.72 &  -4.19 & -4.50 & 3.12\%
    & 16.20 & 11.60 & -3.32 & -2.82 & 6.25\% 
\\
5ggs  & 42.98 & 36.07 & -1.93 & -2.24 & 0\% & 
     17.77 & 7.77 & -5.57 & -6.08 & 12.9\%
\\
4ki5 & 23.81 &  19.74 & -5.19 & -5.47 & 10\%
    &  10.19 & 7.00 & -6.98 & -7.39 & 20\%
\\
4cmh  & 67.89 & 67.11 & 4.99 & 2.47 & 0\%
    &   20.90 & 14.16 & -5.98 & -6.11 & 22.58\%
\\
3hi6  &  48.29 & 47.62 & -1.82 & -1.84 & 0\%
    &  20.21 & 11.83 & -7.71 & -8.01 & 18.75\%
\\
\bottomrule
\end{tabular}

==> tables/success_rate_thresholds.tex <==
\begin{tabular}{c|cccccccccc}
\toprule
       Metric &    95\% &    90\% &   85\% &   80\% &   75\% &   70\% &   65\% &   60\% &   55\% &   50\% \\
\midrule
    CDR $E_{\text{total}}$ & 197.28 & 108.50 & 81.38 & 65.90 & 54.00 & 45.09 & 36.79 & 30.68 & 24.23 & 18.90 \\
    CDR-Ag $\Delta G$ &  17.56 & 3.91 & 0.24 & -0.82 & -2.31 & -3.98 &  -5.34 &  -6.38 & -7.51 & -8.78 \\
\bottomrule
\end{tabular}

==> tables/top1_average_metrics.tex <==
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
     \multirow{2}{*}{Method}
     & \multicolumn{2}{c|}{CDR $E_{\text{total}}$ ($\downarrow$)}
     % & CDR $E_{\text{total}}$ 
     & \multicolumn{2}{c|}{CDR-Ag $E_{\text{nonRep}}$}
     % & CDR-Ag $E_{\text{nonRep}}$
     & \multicolumn{2}{c|}{CDR-Ag $E_{\text{Rep}}$}
     % & CDR-Ag $E_{\text{Rep}}$
     & \multicolumn{2}{c}{CDR-Ag $\Delta G$ ($\downarrow$)}
     % & and CDR-Ag $\Delta G$
     % &  CDR\_avg &  CDR\_med & HsR\_nonRep\_avg & HsR\_nonRep\_med & HsR\_Rep\_avg & HsR\_Rep\_med & HsR\_avg & HsR\_med \\
     \\
     &  Avg. & Med. & Avg. & Med. &  Avg. & Med. & Avg. & Med.  \\
\midrule 
Reference & 4.52 & -1.33 & -17.08 & -18.24 & 6.11 & 4.78 & -13.72 & -14.54 \\
\midrule
   HERN & 7594.94 & 7825.92 &          -6.56 &          -4.57 &     2119.83 &      17.35 & 1159.34 &  4.12 \\
   MEAN &  3113.7 &  2583.48 &          -6.17 &          -4.87 &       220.28 &        3.11 &   114.98 &   -0.92 \\
 dyMEAN & 15025.67 &  7426.40 &         -13.23 &          -7.55 &     4371.34 &      395.29 & 2391.00 &  213.77 \\
dyMEAN* &  3234.30 &  1690.91 &         -13.57 &          -8.86 &     2968.75 &      331.09 & 1619.24 &  177.08 \\
 DiffAb &   211.00 &   155.77 &          -4.82 &          -4.59 &       26.11 &        4.40 &    9.54 &   -1.97 \\
  AbDPO &   162.75 &   124.62 &          -6.90 &          -6.26 &        3.72 &        1.47 &   -4.85 &   -5.24 \\
\bottomrule
\end{tabular}

==> tables/top1_list_result.tex <==
% \renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|rrrr|rrrr|rrrr|rrrr|rrrr|rrrr|rrrr}
\toprule
% \diagbox{Model}{Metric} 


\multirow{3}{*}{PDB id} 
& \multicolumn{4}{c|}{RAbD (Reference)}
& \multicolumn{4}{c|}{HERN}
 & \multicolumn{4}{c|}{MEAN}
  & \multicolumn{4}{c|}{dyMEAN}
  & \multicolumn{4}{c|}{dyMEAN (packed)}
    & \multicolumn{4}{c|}{DiffAb}
        & \multicolumn{4}{c}{\method}
\\

& \multirow{2}{*}{CDR} & HsR & HsR & HsR & \multirow{2}{*}{CDR} & HsR & HsR & HsR & \multirow{2}{*}{CDR} & HsR & HsR & HsR & \multirow{2}{*}{CDR} & HsR & HsR & HsR & \multirow{2}{*}{CDR} & HsR & HsR & HsR & \multirow{2}{*}{CDR} & HsR & HsR & HsR \\
& & Rep & nonRep & Total & & Rep & nonRep & Total & & Rep & nonRep & Total & & Rep & nonRep & Total & & Rep & nonRep & Total & & Rep & nonRep & Total\\
\midrule
  1a14 &    62.28 &           -7.74 &         5.49 &    -4.72 &  5169.68 &           -7.49 &      1646.22 &   897.93 &  4077.06 &           -1.59 &       254.22 &   138.23 &          34174.90 &                    -2.73 &                  0.00 &             -2.73 &           5839.24 &                    -8.77 &               2289.59 &           1250.51 &     152.07 &             -3.40 &           0.42 &      -3.17 &     53.16 &            -5.59 &          1.64 &     -4.69 \\
  1a2y &   -22.18 &           -5.23 &         0.76 &    -4.81 &  6267.55 &           -2.83 &      1486.97 &   815.00 &  2516.51 &           -0.04 &         0.00 &    -0.04 &            451.36 &                     0.04 &                  5.95 &              3.31 &            970.33 &                    -0.44 &                 11.37 &              5.81 &      43.31 &             -3.23 &           0.04 &      -3.20 &     38.51 &            -6.56 &          2.38 &     -5.25 \\
  1fe8 &    25.79 &          -15.73 &         1.61 &   -14.84 &  5399.61 &           -1.20 &         0.45 &    -0.95 &  3615.15 &           -6.75 &       762.74 &   412.76 &            961.32 &                   -16.61 &               2760.42 &           1501.62 &            877.06 &                   -17.96 &               1743.05 &            940.72 &     416.31 &             -8.02 &           3.33 &      -6.19 &    159.14 &            -8.46 &          1.05 &     -7.88 \\
  1ic7 &    19.96 &           -2.86 &         0.43 &    -2.62 &  9436.27 &            4.25 &       258.35 &   146.34 &  1045.54 &            0.42 &         0.00 &     0.42 &            222.66 &                     2.01 &                  0.02 &              2.02 &            185.23 &                    -3.15 &                  5.68 &             -0.02 &       2.97 &             -3.45 &           0.05 &      -3.43 &      3.17 &            -3.00 &          0.00 &     -3.00 \\
  1iqd &    43.36 &          -20.11 &        26.62 &    -5.47 & 10041.48 &           -3.66 &      1051.83 &   574.85 &  2421.77 &          -10.50 &      1713.86 &   932.13 &            334.39 &                    -0.03 &                  0.00 &             -0.03 &           1195.75 &                     0.02 &                  0.00 &              0.02 &     108.52 &             -4.30 &           0.80 &      -3.86 &     25.86 &            -8.18 &          1.46 &     -7.37 \\
  1n8z &    41.88 &          -10.15 &         3.91 &    -8.00 &  5652.93 &          -13.87 &       426.76 &   220.85 &  6601.18 &           -0.02 &         0.10 &     0.04 &          18459.19 &                   -43.32 &              19132.92 &          10479.78 &           5246.39 &                   -43.02 &              15364.78 &           8407.61 &     190.48 &             -8.42 &           2.67 &      -6.95 &    193.26 &            -4.58 &          1.56 &     -3.72 \\
  1ncb &    29.72 &          -18.24 &         6.73 &   -14.54 & 14719.23 &           -8.05 &      3055.98 &  1672.74 &  2260.02 &           -7.13 &      3944.10 &  2162.13 &          14287.93 &                   -18.92 &               2588.12 &           1404.54 &           2653.81 &                   -19.48 &               2336.90 &           1265.82 &     545.06 &              3.72 &         208.27 &     118.26 &    266.65 &            -8.87 &          2.42 &     -7.54 \\
  1osp &    -1.39 &          -18.80 &         5.20 &   -15.94 & 21523.77 &         -154.21 &     72407.16 & 39669.73 &  2587.83 &           -4.80 &       377.83 &   203.00 &          15264.01 &                   -13.57 &               1519.40 &            822.10 &           2066.88 &                   -23.08 &               1267.26 &            673.92 &     253.54 &             -3.12 &           0.86 &      -2.65 &    184.36 &            -8.54 &          3.07 &     -6.85 \\
  1uj3 &   -12.93 &          -13.33 &         3.41 &   -11.45 & 12510.05 &            0.93 &         0.25 &     1.06 &  5358.69 &            0.27 &         3.58 &     2.24 &            296.24 &                    -1.27 &                237.64 &            129.43 &            318.82 &                    -3.84 &                105.50 &             54.18 &     127.33 &             -7.73 &           6.61 &      -4.10 &    115.91 &            -4.44 &          0.98 &     -3.90 \\
  1w72 &     7.24 &          -18.65 &         4.71 &   -16.06 & 11403.26 &           -6.23 &       243.95 &   127.94 &  3760.71 &           -1.89 &       235.99 &   127.91 &          19427.87 &                    -0.34 &                  0.00 &             -0.34 &           5197.96 &                    -1.34 &                  5.34 &              1.60 &     218.04 &              2.21 &         143.75 &      81.27 &    136.72 &            -3.51 &          1.67 &     -2.59 \\
  2adf &   -20.47 &          -20.95 &         9.87 &   -15.53 &  9945.88 &          -17.06 &      3343.58 &  1821.91 &  3986.81 &          -23.00 &      3086.52 &  1674.59 &           4598.94 &                   -25.54 &               3811.31 &           2070.68 &           2079.50 &                   -21.50 &               2275.87 &           1230.23 &     129.37 &             -8.94 &           6.17 &      -5.54 &    151.56 &           -13.90 &          3.25 &    -12.11 \\
  2b2x &     2.45 &           -7.91 &         1.99 &    -6.81 &  8224.51 &           -5.67 &      1955.48 &  1069.85 &  2927.38 &           -2.03 &       742.31 &   406.24 &            633.94 &                    -1.82 &                145.38 &             78.14 &            359.68 &                    -2.30 &                126.03 &             67.01 &     419.03 &             -3.31 &           0.25 &      -3.17 &    202.22 &            -6.78 &          1.47 &     -5.97 \\
  2cmr &     5.14 &          -11.72 &         3.51 &    -9.79 & 14457.07 &          -28.25 &      2657.26 &  1433.24 &  2216.17 &          -10.86 &      3145.14 &  1718.96 &            888.96 &                    -7.74 &               2559.44 &           1399.95 &            680.68 &                   -11.50 &               1713.09 &            930.70 &     214.32 &             -7.24 &          24.71 &       6.36 &    791.54 &           -10.60 &         30.31 &      6.07 \\
  2dd8 &    68.27 &           -9.27 &         1.00 &    -8.72 & 10213.29 &          -13.25 &      4443.14 &  2430.47 &  2860.40 &           -5.33 &        60.21 &    27.78 &            733.46 &                    -2.52 &               1002.66 &            548.94 &           1309.13 &                    -9.40 &               2143.32 &           1169.43 &      78.03 &             -7.12 &           0.88 &      -6.64 &     17.73 &            -3.54 &          2.33 &     -2.26 \\
  2vxt &   -10.32 &          -15.66 &         4.93 &   -12.95 &  5023.30 &           -0.64 &         0.00 &    -0.64 &  1738.42 &            9.56 &       978.49 &   547.73 &            191.82 &                    -0.88 &                 15.36 &              7.56 &            350.35 &                    -3.42 &                 17.98 &              6.47 &      18.08 &             -6.99 &           4.50 &      -4.51 &     32.77 &            -3.96 &          0.73 &     -3.55 \\
  2xqy &    -3.67 &          -19.16 &         5.50 &   -16.14 &  9818.37 &           -1.33 &       585.42 &   320.66 &  1361.69 &           -2.69 &        64.25 &    32.64 &           4953.36 &                   -16.52 &               2965.11 &           1614.29 &           2980.74 &                   -22.63 &               4448.85 &           2424.24 &     123.55 &            -14.09 &           8.06 &      -9.65 &     41.48 &            -9.08 &          0.68 &     -8.71 \\
  2xwt &   -19.96 &          -30.62 &         4.78 &   -27.99 & 14372.97 &          -13.84 &      4616.06 &  2525.00 &  1171.72 &           -5.67 &       437.83 &   235.14 &          11202.50 &                    -7.15 &               2685.05 &           1469.63 &           1758.57 &                    -7.70 &               1226.06 &            666.63 &     523.87 &             -3.51 &           5.15 &      -0.68 &    133.26 &            -8.94 &          5.55 &     -5.88 \\
  2ypv &     4.72 &           -8.36 &         2.59 &    -6.94 & 15668.71 &           -3.39 &       372.84 &   201.67 &  2999.63 &            0.89 &       656.29 &   361.85 &           7482.75 &                   -11.74 &               3727.40 &           2038.33 &           3083.17 &                    -3.82 &               2978.32 &           1634.25 &     257.76 &              2.61 &           9.06 &       7.59 &     59.37 &            -5.65 &          0.15 &     -5.57 \\
  3bn9 &    81.99 &           -0.92 &         0.05 &    -0.89 & 12755.52 &           -7.53 &      2764.09 &  1512.72 &  6552.67 &           -0.76 &         0.00 &    -0.76 &           3736.29 &                   -11.53 &              12928.34 &           7099.06 &           2313.10 &                   -11.66 &               8151.58 &           4471.70 &     304.96 &             -2.21 &           0.42 &      -1.98 &    238.62 &            -5.73 &          1.35 &     -4.99 \\
  3cx5 &   -18.25 &          -19.29 &         7.98 &   -14.91 & 15747.06 &           -7.06 &      1109.95 &   603.41 &  7041.64 &            0.93 &        23.78 &    14.01 &           4471.76 &                    -2.46 &                373.62 &            203.03 &           1310.86 &                    -7.09 &                468.17 &            250.40 &     223.68 &             -9.61 &           7.40 &      -5.54 &     64.67 &            -8.42 &          4.07 &     -6.18 \\
  3ffd &    43.13 &          -17.23 &         8.37 &   -12.63 &  3029.53 &          -10.61 &      1468.34 &   796.97 &  3121.12 &          -10.60 &       112.30 &    51.16 &           8216.38 &                   -40.44 &              12836.40 &           7019.58 &           2734.41 &                   -31.29 &               7330.08 &           4000.26 &     156.48 &            -10.13 &         109.86 &      50.29 &    394.04 &           -15.00 &          8.09 &    -10.55 \\
  3hi6 &   -12.57 &          -40.73 &        12.00 &   -34.13 & 11107.88 &           -2.37 &         3.20 &    -0.61 &  5499.23 &          -21.18 &      2321.29 &  1255.53 &           4117.88 &                    -2.48 &                  5.43 &              0.51 &           1113.78 &                    -0.90 &                  1.43 &             -0.12 &     416.34 &             -4.28 &          15.45 &       4.22 &    248.63 &            -7.94 &          2.43 &     -6.61 \\
  3k2u &    18.71 &          -19.21 &         8.44 &   -14.57 & 11168.20 &           -0.21 &       237.14 &   130.22 &  2362.96 &          -12.51 &      2897.57 &  1581.15 &          10703.42 &                   -32.99 &              19333.55 &          10600.46 &           4418.98 &                   -38.22 &              13858.01 &           7583.69 &      99.64 &             -2.14 &          24.95 &      11.59 &    417.20 &            -8.11 &          3.29 &     -6.30 \\
  3l95 &    -1.24 &          -20.02 &         2.80 &   -18.48 & 17510.86 &          -18.69 &      2560.68 &  1389.69 &  3539.90 &           -8.52 &       520.56 &   277.79 &           8077.74 &                   -30.63 &               2808.87 &           1514.25 &           2675.90 &                   -38.44 &               5014.83 &           2719.71 &     155.07 &             -5.38 &           6.74 &      -1.68 &    263.98 &            -5.90 &          1.21 &     -5.24 \\
  3mxw &    -6.64 &          -18.76 &         2.81 &   -17.22 &  8220.08 &            2.60 &        82.47 &    47.96 &  3584.58 &           -8.07 &      3675.78 &  2013.61 &           7689.73 &                    -0.82 &               2239.50 &           1230.90 &           2092.64 &                    -8.99 &               1367.24 &            742.99 &      62.73 &              1.26 &          24.46 &      14.71 &    129.19 &            -4.29 &          0.34 &     -4.11 \\
  3nid &   -21.55 &          -35.71 &         8.65 &   -30.95 & 11220.75 &           -9.55 &      1483.10 &   806.16 &  5147.42 &          -18.91 &      1850.81 &   999.04 &           7746.78 &                   -19.71 &                862.71 &            454.78 &           1321.36 &                   -12.35 &                 70.39 &             26.37 &     305.98 &             -3.42 &          89.07 &      45.57 &     96.66 &            -9.14 &         69.47 &     29.06 \\
  3o2d &     0.23 &          -19.46 &        10.99 &   -13.42 &  6691.29 &          -10.73 &      1532.45 &   832.12 & 12914.73 &          -11.83 &      3778.56 &  2066.38 &          40369.25 &                   -29.57 &               8834.98 &           4829.67 &           7384.70 &                   -26.90 &               3083.24 &           1668.88 &     165.05 &             -1.88 &           0.19 &      -1.77 &    138.54 &            -5.21 &          1.89 &     -4.17 \\
  3rkd &    -6.61 &          -14.88 &         8.24 &   -10.35 &  3879.97 &           -5.75 &       550.50 &   297.03 &  4566.02 &           -8.45 &      1326.56 &   721.15 &          14966.23 &                     0.45 &                  0.00 &              0.45 &           2965.58 &                     1.59 &                 12.65 &              8.55 &     418.45 &             -6.37 &           4.29 &      -4.01 &     88.66 &            -9.51 &          0.39 &     -9.30 \\
  3s35 &   -16.27 &           -7.94 &         4.26 &    -5.60 &  7790.91 &            2.66 &      2210.25 &  1218.30 &  3192.78 &           -6.73 &         0.80 &    -6.28 &            321.14 &                    -4.71 &                528.27 &            285.84 &            279.15 &                    -8.52 &                145.73 &             71.63 &      39.79 &             -5.34 &           3.64 &      -3.34 &     22.03 &            -4.98 &          0.66 &     -4.61 \\
  3w9e &    -9.93 &          -26.05 &         6.20 &   -22.64 & 17894.72 &          -21.64 &      7698.87 &  4212.74 &  4512.84 &          -11.99 &       961.93 &   517.07 &          45707.54 &                   -96.89 &              58688.75 &          32181.92 &          17178.60 &                   -88.46 &              46545.61 &          25511.63 &     277.09 &             -7.74 &          11.29 &      -1.53 &    143.46 &            -7.15 &          2.32 &     -5.87 \\
  4cmh &   -19.18 &          -19.86 &         6.02 &   -16.54 &  8710.74 &           -8.39 &      1162.27 &   630.86 &  6040.00 &          -20.59 &      6149.58 &  3361.68 &          15710.26 &                   -19.65 &               1109.65 &            590.66 &           4516.38 &                   -17.56 &               7301.71 &           3998.38 &     504.03 &             -3.17 &         341.51 &     184.67 &    145.62 &            -4.92 &          2.24 &     -3.69 \\
  4dtg &     6.29 &           -8.93 &         6.36 &    -5.43 & 12467.03 &          -50.94 &     41317.70 & 22673.79 &  7327.45 &           -0.25 &        39.63 &    21.55 &          28678.84 &                    -4.98 &               1654.15 &            904.80 &           2095.90 &                    -7.22 &               2200.30 &           1202.94 &     111.13 &             -4.81 &          19.40 &       5.86 &     83.31 &            -7.64 &          4.29 &     -5.28 \\
  4dvr &    -6.74 &           -0.13 &         2.29 &     1.13 & 10563.25 &           -6.09 &         9.33 &    -0.95 &  5541.72 &           -8.97 &        55.65 &    21.64 &           6658.80 &                   -21.29 &               5580.01 &           3047.72 &           1584.51 &                   -23.91 &               3780.43 &           2055.33 &     139.59 &             -6.65 &           2.59 &      -5.22 &     53.45 &            -6.75 &          4.80 &     -4.11 \\
  4ffv &    28.69 &           -0.69 &         2.47 &     0.67 &  2965.17 &           -0.60 &         0.00 &    -0.60 &  2074.62 &           -0.41 &         0.00 &    -0.41 &            338.75 &                    -2.41 &                  0.09 &             -2.36 &           1768.83 &                    -2.40 &                  0.09 &             -2.35 &      70.33 &             -3.42 &           1.93 &      -2.36 &     40.20 &            -1.63 &          0.34 &     -1.44 \\
  4fqj &    33.50 &          -31.89 &        18.12 &   -21.93 & 17261.80 &           -2.42 &       408.84 &   222.45 &  3845.64 &           -7.95 &      1161.37 &   630.81 &          45248.70 &                    -1.00 &                 51.60 &             27.38 &           9408.77 &                    -1.51 &               1636.47 &            898.55 &     353.39 &             -5.71 &          33.95 &      12.96 &    617.51 &           -10.70 &          0.48 &    -10.44 \\
  4g6j &     0.30 &          -10.77 &         3.56 &    -8.81 & 13799.45 &            3.37 &      1043.86 &   577.49 &  2958.05 &           -3.76 &      1262.75 &   690.75 &           3123.66 &                    -3.14 &                850.72 &            464.75 &            639.37 &                   -12.05 &               1157.63 &            624.65 &     128.27 &             -0.49 &           0.60 &      -0.16 &     67.11 &            -3.80 &          1.45 &     -3.00 \\
  4g6m &    -8.60 &          -23.53 &         3.48 &   -21.61 &  7880.16 &           -9.43 &       857.49 &   462.19 &  4797.36 &           -3.13 &       140.17 &    73.97 &           7164.21 &                   -27.12 &              11460.91 &           6276.39 &           3012.94 &                   -30.02 &               8827.56 &           4825.13 &      28.07 &             -6.08 &           1.57 &      -5.22 &      8.07 &            -6.45 &          0.44 &     -6.21 \\
  4h8w &    -1.33 &          -15.91 &         3.23 &   -14.14 & 11854.24 &           -1.65 &         0.29 &    -1.49 &  2469.34 &            3.31 &       942.08 &   521.46 &           8791.56 &                   -17.68 &               3814.83 &           2080.47 &           1306.59 &                   -24.26 &               3643.64 &           1979.74 &     112.21 &             -6.52 &          12.46 &       0.33 &    131.44 &            -8.50 &          6.17 &     -5.11 \\
  4ki5 &    -8.15 &          -19.54 &         5.37 &   -16.58 &  3749.11 &           -9.46 &      1041.45 &   563.33 &  6183.14 &            5.46 &      2064.39 &  1140.87 &          35711.59 &                    -8.80 &                  7.98 &             -4.41 &           3303.49 &                   -20.75 &               1956.46 &           1055.30 &     166.79 &             -1.80 &           0.04 &      -1.78 &     76.98 &            -6.05 &          0.58 &     -5.73 \\
  4lvn &    40.37 &          -16.18 &         8.34 &   -11.59 &  9069.95 &           -3.14 &       293.24 &   158.14 &  4439.20 &           -0.86 &         0.38 &    -0.65 &          29120.62 &                   -79.77 &              58557.77 &          32127.00 &          14497.16 &                   -81.81 &              45581.07 &          24987.79 &     504.98 &             -3.60 &           0.94 &      -3.09 &    177.60 &            -4.88 &          0.73 &     -4.48 \\
  4ot1 &   -13.23 &          -30.77 &         9.09 &   -25.77 &  7065.27 &            4.18 &      1131.41 &   626.46 & 19673.69 &          -27.72 &     12239.66 &  6704.09 &         132049.55 &                    -0.13 &                  0.00 &             -0.13 &          26820.86 &                     2.57 &                 15.23 &             10.95 &     178.79 &             -8.48 &          48.30 &      18.09 &    157.70 &            -4.40 &          0.01 &     -4.39 \\
  4qci &     5.68 &           -3.37 &         0.04 &    -3.35 &  3138.14 &           -0.75 &      1716.82 &   943.50 &  2337.96 &           -0.00 &         0.00 &    -0.00 &           7458.94 &                    -0.37 &                  0.00 &             -0.37 &            580.91 &                     1.13 &                 10.52 &              6.92 &      82.63 &             -2.29 &           0.04 &      -2.27 &     35.99 &            -2.01 &          0.16 &     -1.92 \\
  4xnq &   -18.37 &          -23.84 &         5.38 &   -20.88 & 12941.26 &          -23.77 &      2136.96 &  1151.55 &  8013.93 &          -22.19 &      3394.18 &  1844.61 &          25335.47 &                    -1.26 &                  0.01 &             -1.26 &           4541.00 &                    -5.27 &               1378.36 &            752.83 &     282.80 &             -5.04 &           5.99 &      -1.74 &    117.00 &            -4.95 &          0.01 &     -4.94 \\
  4ydk &   -31.29 &          -38.30 &         7.69 &   -34.08 & 23424.95 &           -3.31 &         8.14 &     1.17 & 14293.06 &          -39.00 &     13584.27 &  7432.35 &          69556.07 &                    -0.63 &                  0.00 &             -0.63 &          14781.14 &                    -1.82 &                  6.03 &              1.50 &     593.74 &              5.84 &          31.03 &      22.91 &    915.51 &           -12.33 &          9.63 &     -7.04 \\
  5b8c &    -4.19 &          -21.12 &        10.70 &   -15.23 &  4473.90 &          -13.90 &       391.94 &   201.67 &  2864.55 &           -4.65 &        11.66 &     1.77 &          10547.32 &                    -6.08 &                  1.45 &             -5.28 &           1790.96 &                   -24.63 &               1955.54 &           1050.92 &      56.26 &             -6.49 &           1.66 &      -5.57 &    118.91 &            -7.53 &          2.61 &     -6.09 \\
  5bv7 &    44.87 &          -39.40 &        38.47 &   -18.25 & 13358.66 &          -47.63 &      9581.93 &  5222.43 &  8913.90 &          -27.88 &      2270.36 &  1220.81 &          64586.68 &                   -41.32 &              20501.67 &          11234.60 &          14429.15 &                   -26.48 &               5912.41 &           3225.35 &     214.86 &            -13.48 &          80.05 &      30.54 &    277.37 &            -5.08 &          3.23 &     -3.30 \\
  5d93 &    -6.28 &           -7.43 &         1.10 &    -6.83 & 11797.74 &           -4.78 &       288.42 &   153.85 &  3285.86 &           -3.28 &        23.65 &     9.73 &           2219.78 &                   -13.55 &               5402.21 &           2957.67 &           1010.38 &                    -8.40 &                 24.70 &              5.18 &      48.56 &             -4.38 &           0.62 &      -4.04 &     64.57 &            -5.66 &          0.76 &     -5.25 \\
  5en2 &   -20.91 &          -12.80 &         5.68 &    -9.67 & 14790.23 &           -9.81 &      3219.60 &  1760.97 &  7265.91 &          -18.81 &      4203.77 &  2293.26 &          48703.53 &                   -15.18 &                520.22 &            270.94 &          10080.22 &                   -27.45 &               2094.45 &           1124.50 &     476.51 &            -10.44 &          35.10 &       8.86 &     87.25 &            -4.97 &          0.17 &     -4.87 \\
  5f9o &     5.96 &          -17.28 &         2.04 &   -16.16 &  5396.01 &           12.57 &      1420.64 &   793.92 &  2997.97 &          -18.19 &      3424.07 &  1865.04 &          20163.27 &                    -4.09 &                 16.95 &              5.23 &           3281.56 &                   -10.61 &               2957.68 &           1616.11 &     147.07 &             -0.76 &           1.09 &      -0.17 &    168.54 &            -4.25 &          0.04 &     -4.22 \\
  5ggs &   -15.18 &          -21.95 &         7.63 &   -17.75 &  6832.37 &          -11.29 &      1462.35 &   793.01 &  3935.96 &           -7.72 &       125.74 &    61.44 &          14681.00 &                     1.38 &               2820.06 &           1552.41 &           1240.98 &                   -10.60 &                962.00 &            518.50 &      94.70 &             -5.53 &           0.69 &      -5.15 &     71.94 &            -9.61 &          1.09 &     -9.01 \\
  5hi4 &     0.48 &          -20.27 &         4.00 &   -18.07 & 11598.05 &          -66.92 &     32613.24 & 17870.36 &  4673.60 &          -13.25 &       451.73 &   235.21 &           2573.00 &                   -40.80 &               7491.10 &           4079.31 &           2584.78 &                   -32.45 &               8064.11 &           4402.80 &     108.56 &             -3.95 &           1.05 &      -3.37 &    152.57 &            -9.42 &          2.82 &     -7.87 \\
  5j13 &     0.61 &          -19.75 &         1.79 &   -18.76 & 10742.92 &           -6.12 &      9445.26 &  5188.77 &  7892.10 &            0.84 &       131.99 &    73.43 &          25803.23 &                     0.02 &                 63.59 &             34.99 &           1907.72 &                    -2.17 &                  0.01 &             -2.17 &     106.87 &             -1.24 &           0.60 &      -0.91 &    140.27 &            -6.07 &          0.55 &     -5.77 \\
  5l6y &    -0.46 &          -12.26 &         3.31 &   -10.43 & 19579.00 &          -15.56 &      2311.92 &  1256.00 &  4210.93 &           -9.23 &      1926.48 &  1050.33 &          27092.55 &                   -11.07 &                133.91 &             62.58 &           1596.31 &                    -4.11 &                  6.81 &             -0.37 &      64.99 &             -3.34 &           1.09 &      -2.75 &    194.99 &            -5.62 &          1.62 &     -4.73 \\
  5mes &   -16.95 &           -9.16 &         3.17 &    -7.42 &  9270.86 &           -3.89 &       104.10 &    53.36 &  2882.11 &           -1.10 &         0.00 &    -1.10 &           4487.38 &                    -3.36 &                 11.57 &              3.00 &            826.24 &                    -4.46 &                985.46 &            537.54 &     123.85 &             -7.40 &           0.96 &      -6.87 &     74.85 &           -12.49 &          3.20 &    -10.73 \\
  5nuz &   -18.37 &          -19.79 &         2.90 &   -18.19 & 16269.67 &          -17.68 &      1938.60 &  1048.55 &  3092.27 &          -12.85 &       117.11 &    51.56 &          18080.87 &                   -64.48 &              18517.68 &          10120.25 &           6520.63 &                   -58.00 &              13857.01 &           7563.36 &     459.22 &            -14.15 &          89.50 &      35.07 &    120.05 &            -8.10 &          1.13 &     -7.48 \\
\bottomrule
\end{tabular}
% \renewcommand{\arraystretch}{1}

==> tables/top1_list_result_long.tex <==
{\tiny
% Reduce the font size
\setlength{\tabcolsep}{2pt} % Reduce the column separation
% \renewcommand{\arraystretch}{1.2}
\begin{longtable}{c|rrrr|rrrr|rrrr|rrrr|rrrr|rrrr|rrrr}
\caption{Detailed evaluation results for reference antibodies and antibodies designed by HERN, MEAN, dyMEAN, dymean (packed), DiffAb, and \method for 55 antigens. The data source is the same as that in \cref{tab:main_result}. For simplicity, we use A,B,C, and D to stand for CDR $E_{\text{total}}$. CDR-Ag $E_{\text{nonRep}}$, CDR-Ag $E_{\text{Rep}}$, and CDR-Ag $\Delta G$ respectively in this table. The unit is kcal/mol and omitted for brevity.}\label{tab:top1_list_result_long}
\endfirsthead
\endhead
\toprule
% \diagbox{Model}{Metric} 


\multirow{2}{*}{PDB id} 
& \multicolumn{4}{c|}{RAbD (Reference)}
& \multicolumn{4}{c|}{HERN}
 & \multicolumn{4}{c|}{MEAN}
  & \multicolumn{4}{c|}{dyMEAN}
  & \multicolumn{4}{c|}{dyMEAN (packed)}
    & \multicolumn{4}{c|}{DiffAb}
        & \multicolumn{4}{c}{\method}
\\
% & CDR & $E_{\text{nonRep}}$ & $E_{\text{Rep}}$ &  $\Delta G$ & CDR & CDR-Ag & CDR-Ag & CDR-Ag& CDR & CDR-Ag & CDR-Ag & CDR-Ag& CDR & CDR-Ag & CDR-Ag & CDR-Ag& CDR & CDR-Ag & CDR-Ag & CDR-Ag& CDR & CDR-Ag & CDR-Ag & CDR-Ag \\
% & & Rep & nonRep & Total & & Rep & nonRep & Total & & Rep & nonRep & Total & & Rep & nonRep & Total & & Rep & nonRep & Total & & Rep & nonRep & Total\\
& A&B&C&D& A&B&C&D& A&B&C&D& A&B&C&D& A&B&C&D & A&B&C&D& A&B&C&D\\
\midrule
  1a14 &    62.28 &           -7.74 &         5.49 &    -4.72 &  3305.94 &           -5.24 &         1.69 &    -4.31 &  4234.38 &           -6.06 &         2.98 &    -4.42 &          32183.85 &                    -3.47 &                  0.01 &             -3.47 &           5465.48 &                    -6.74 &                 13.21 &              0.53 &     152.07 &             -3.40 &           0.42 &      -3.17 &     53.16 &            -5.59 &          1.64 &     -4.69 \\
  1a2y &   -22.18 &           -5.23 &         0.76 &    -4.81 &  5833.44 &           -2.44 &         0.13 &    -2.37 &   620.01 &           -2.51 &         1.72 &    -1.57 &            416.51 &                    -0.80 &                  3.11 &              0.91 &            739.56 &                    -0.93 &                  4.16 &              1.35 &      43.31 &             -3.23 &           0.04 &      -3.20 &     38.51 &            -6.56 &          2.38 &     -5.25 \\
  1fe8 &    25.79 &          -15.73 &         1.61 &   -14.84 &  2692.37 &           -4.08 &         1.73 &    -3.13 &  1559.74 &          -12.08 &        24.75 &     1.53 &            587.40 &                   -14.50 &               1255.78 &            676.18 &            206.67 &                    -8.99 &                249.51 &            128.24 &     416.31 &             -8.02 &           3.33 &      -6.19 &    159.14 &            -8.46 &          1.05 &     -7.88 \\
  1ic7 &    19.96 &           -2.86 &         0.43 &    -2.62 &  3996.06 &           -5.71 &         2.23 &    -4.48 &   550.68 &           -4.92 &         0.22 &    -4.80 &            216.02 &                     1.62 &                  0.01 &              1.62 &            179.52 &                    -2.94 &                  3.81 &             -0.84 &       2.97 &             -3.45 &           0.05 &      -3.43 &      3.17 &            -3.00 &          0.00 &     -3.00 \\
  1iqd &    43.36 &          -20.11 &        26.62 &    -5.47 &  8090.59 &           -2.46 &         0.08 &    -2.41 &   986.12 &           -3.09 &         0.00 &    -3.09 &            314.47 &                    -0.10 &                  0.00 &             -0.10 &           1085.70 &                    -0.00 &                  0.00 &             -0.00 &     108.52 &             -4.30 &           0.80 &      -3.86 &     25.86 &            -8.18 &          1.46 &     -7.37 \\
  1n8z &    41.88 &          -10.15 &         3.91 &    -8.00 &  4256.36 &          -12.16 &        18.45 &    -2.01 &  2228.64 &            0.15 &         0.17 &     0.24 &          14653.75 &                   -36.72 &              13967.83 &           7645.58 &           3344.40 &                   -27.49 &               8720.51 &           4768.79 &     190.48 &             -8.42 &           2.67 &      -6.95 &    193.26 &            -4.58 &          1.56 &     -3.72 \\
  1ncb &    29.72 &          -18.24 &         6.73 &   -14.54 & 13169.66 &           -3.01 &        29.37 &    13.14 &  1877.43 &           -5.56 &       801.72 &   435.39 &          12631.40 &                   -16.76 &               1719.62 &            929.03 &           2426.56 &                   -17.91 &               1724.04 &            930.32 &     545.06 &              3.72 &         208.27 &     118.26 &    266.65 &            -8.87 &          2.42 &     -7.54 \\
  1osp &    -1.39 &          -18.80 &         5.20 &   -15.94 & 15897.17 &         -105.29 &     53075.05 & 29085.99 &  1593.02 &           -7.99 &        59.47 &    24.72 &          13908.80 &                   -11.75 &               1113.40 &            600.62 &           1801.60 &                   -19.76 &                612.21 &            316.95 &     253.54 &             -3.12 &           0.86 &      -2.65 &    184.36 &            -8.54 &          3.07 &     -6.85 \\
  1uj3 &   -12.93 &          -13.33 &         3.41 &   -11.45 & 10353.51 &           -1.93 &         0.85 &    -1.46 &  1714.56 &           -3.64 &         2.88 &    -2.06 &            232.72 &                    -3.58 &                  0.76 &             -3.17 &            283.31 &                    -4.03 &                  1.04 &             -3.46 &     127.33 &             -7.73 &           6.61 &      -4.10 &    115.91 &            -4.44 &          0.98 &     -3.90 \\
  1w72 &     7.24 &          -18.65 &         4.71 &   -16.06 &  9182.60 &           -4.10 &        23.49 &     8.82 &  2109.58 &           -1.82 &         0.02 &    -1.81 &          18104.26 &                    -0.49 &                  0.00 &             -0.49 &           4664.74 &                    -0.04 &                  0.00 &             -0.04 &     218.04 &              2.21 &         143.75 &      81.27 &    136.72 &            -3.51 &          1.67 &     -2.59 \\
  2adf &   -20.47 &          -20.95 &         9.87 &   -15.53 &  7275.04 &           -5.69 &         2.91 &    -4.09 &  2757.71 &           -8.09 &       187.02 &    94.77 &           4230.05 &                   -21.07 &               2850.68 &           1546.81 &            368.12 &                   -13.12 &                557.50 &            293.51 &     129.37 &             -8.94 &           6.17 &      -5.54 &    151.56 &           -13.90 &          3.25 &    -12.11 \\
  2b2x &     2.45 &           -7.91 &         1.99 &    -6.81 &  6735.92 &           -7.52 &         4.31 &    -5.15 &  4816.48 &          -10.47 &        11.82 &    -3.97 &            593.02 &                    -2.20 &                 39.19 &             19.35 &            287.23 &                    -2.60 &                 31.70 &             14.84 &     419.03 &             -3.31 &           0.25 &      -3.17 &    202.22 &            -6.78 &          1.47 &     -5.97 \\
  2cmr &     5.14 &          -11.72 &         3.51 &    -9.79 &  8971.08 &           -9.12 &       138.66 &    67.14 &  3787.78 &           -8.20 &         1.43 &    -7.42 &            446.95 &                   -10.43 &                959.08 &            517.07 &            406.96 &                   -11.21 &                954.56 &            513.80 &     214.32 &             -7.24 &          24.71 &       6.36 &    791.54 &           -10.60 &         30.31 &      6.07 \\
  2dd8 &    68.27 &           -9.27 &         1.00 &    -8.72 &  7313.83 &           -9.27 &        17.35 &     0.27 &  3266.95 &           -6.66 &         6.04 &    -3.34 &            589.27 &                    -3.64 &                395.29 &            213.77 &            896.01 &                    -6.65 &                719.48 &            389.07 &      78.03 &             -7.12 &           0.88 &      -6.64 &     17.73 &            -3.54 &          2.33 &     -2.26 \\
  2vxt &   -10.32 &          -15.66 &         4.93 &   -12.95 &  3627.03 &           -1.73 &         0.00 &    -1.73 &   728.65 &           -2.31 &         1.30 &    -1.60 &            162.33 &                    -0.85 &                  3.96 &              1.33 &            213.46 &                    -3.46 &                  2.75 &             -1.95 &      18.08 &             -6.99 &           4.50 &      -4.51 &     32.77 &            -3.96 &          0.73 &     -3.55 \\
  2xqy &    -3.67 &          -19.16 &         5.50 &   -16.14 &  9260.53 &           -1.47 &         0.56 &    -1.17 &   557.94 &           -4.70 &         6.35 &    -1.21 &           4586.60 &                   -12.24 &               2374.31 &           1293.63 &           1323.92 &                   -12.55 &                 92.77 &             38.47 &     123.55 &            -14.09 &           8.06 &      -9.65 &     41.48 &            -9.08 &          0.68 &     -8.71 \\
  2xwt &   -19.96 &          -30.62 &         4.78 &   -27.99 &  9805.20 &           -1.51 &         0.07 &    -1.47 &  2536.40 &          -11.21 &       303.02 &   155.44 &          10760.25 &                    -7.55 &               1844.76 &           1007.06 &           1609.46 &                    -7.29 &               1014.33 &            550.58 &     523.87 &             -3.51 &           5.15 &      -0.68 &    133.26 &            -8.94 &          5.55 &     -5.88 \\
  2ypv &     4.72 &           -8.36 &         2.59 &    -6.94 & 13302.47 &           -4.88 &        58.55 &    27.32 &  2583.48 &            0.38 &      1889.09 &  1039.38 &           6716.63 &                    -9.71 &               1966.02 &           1071.60 &           1045.60 &                   -16.07 &               2247.75 &           1220.19 &     257.76 &              2.61 &           9.06 &       7.59 &     59.37 &            -5.65 &          0.15 &     -5.57 \\
  3bn9 &    81.99 &           -0.92 &         0.05 &    -0.89 & 10227.13 &           -1.33 &         0.49 &    -1.06 &  3109.87 &           -3.64 &         1.90 &    -2.59 &           3526.68 &                   -10.18 &              12194.28 &           6696.68 &           2039.29 &                    -9.93 &               7142.17 &           3918.27 &     304.96 &             -2.21 &           0.42 &      -1.98 &    238.62 &            -5.73 &          1.35 &     -4.99 \\
  3cx5 &   -18.25 &          -19.29 &         7.98 &   -14.91 & 13087.27 &           -4.77 &       496.31 &   268.20 &  3405.67 &           -5.13 &         0.58 &    -4.81 &           3909.41 &                    -2.90 &                147.98 &             78.49 &            946.84 &                    -5.97 &                272.73 &            144.04 &     223.68 &             -9.61 &           7.40 &      -5.54 &     64.67 &            -8.42 &          4.07 &     -6.18 \\
  3ffd &    43.13 &          -17.23 &         8.37 &   -12.63 &  1657.51 &           -7.43 &         0.86 &    -6.96 &  1124.49 &           -4.20 &         2.89 &    -2.61 &           7426.40 &                   -41.49 &              11643.08 &           6362.20 &           1924.13 &                   -35.90 &               5086.41 &           2761.62 &     156.48 &            -10.13 &         109.86 &      50.29 &    394.04 &           -15.00 &          8.09 &    -10.55 \\
  3hi6 &   -12.57 &          -40.73 &        12.00 &   -34.13 & 10584.20 &           -9.15 &         5.54 &    -6.10 &  6232.66 &          -21.33 &      1328.42 &   709.30 &            409.24 &                    -1.18 &                  1.25 &             -0.49 &            866.23 &                    -1.06 &                  0.70 &             -0.67 &     416.34 &             -4.28 &          15.45 &       4.22 &    248.63 &            -7.94 &          2.43 &     -6.61 \\
  3k2u &    18.71 &          -19.21 &         8.44 &   -14.57 &  8004.09 &           -2.93 &         0.03 &    -2.92 &  2914.51 &           -6.92 &      1455.45 &   793.58 &           9822.96 &                   -27.58 &              16858.37 &           9244.53 &           2438.16 &                   -23.09 &               5482.50 &           2992.28 &      99.64 &             -2.14 &          24.95 &      11.59 &    417.20 &            -8.11 &          3.29 &     -6.30 \\
  3l95 &    -1.24 &          -20.02 &         2.80 &   -18.48 & 11740.49 &           -3.81 &         0.94 &    -3.29 &  3194.42 &          -10.69 &        44.28 &    13.66 &           3456.71 &                   -25.96 &               1142.97 &            602.67 &           1176.11 &                   -35.11 &               2006.60 &           1068.52 &     155.07 &             -5.38 &           6.74 &      -1.68 &    263.98 &            -5.90 &          1.21 &     -5.24 \\
  3mxw &    -6.64 &          -18.76 &         2.81 &   -17.22 &  6308.62 &            2.67 &         0.15 &     2.75 &  2088.31 &           -1.76 &         8.47 &     2.89 &           7270.76 &                     1.69 &                919.22 &            507.26 &           1741.92 &                    -5.02 &                331.09 &            177.08 &      62.73 &              1.26 &          24.46 &      14.71 &    129.19 &            -4.29 &          0.34 &     -4.11 \\
  3nid &   -21.55 &          -35.71 &         8.65 &   -30.95 &  7098.49 &           -1.61 &        61.68 &    32.31 &  5791.62 &          -21.02 &      2911.12 &  1580.10 &           7537.68 &                   -18.50 &                617.18 &            320.95 &           1130.19 &                   -11.68 &                 31.77 &              5.80 &     305.98 &             -3.42 &          89.07 &      45.57 &     96.66 &            -9.14 &         69.47 &     29.06 \\
  3o2d &     0.23 &          -19.46 &        10.99 &   -13.42 &  3017.40 &           -8.88 &      1006.06 &   544.45 &  4605.52 &           -4.81 &         1.63 &    -3.92 &          30284.96 &                   -19.83 &               2702.77 &           1466.69 &           4746.20 &                    -9.66 &                955.21 &            515.71 &     165.05 &             -1.88 &           0.19 &      -1.77 &    138.54 &            -5.21 &          1.89 &     -4.17 \\
  3rkd &    -6.61 &          -14.88 &         8.24 &   -10.35 &  1822.10 &           -4.26 &        74.75 &    36.85 &  2291.36 &           -4.87 &         0.85 &    -4.40 &          14090.88 &                     0.28 &                  0.00 &              0.28 &           2637.93 &                     0.29 &                  3.78 &              2.37 &     418.45 &             -6.37 &           4.29 &      -4.01 &     88.66 &            -9.51 &          0.39 &     -9.30 \\
  3s35 &   -16.27 &           -7.94 &         4.26 &    -5.60 &  5224.56 &           -4.54 &        11.87 &     1.99 &  1429.28 &          -12.17 &       104.95 &    45.55 &            192.59 &                    -0.27 &                  0.00 &             -0.27 &            242.69 &                    -3.34 &                  0.00 &             -3.34 &      39.79 &             -5.34 &           3.64 &      -3.34 &     22.03 &            -4.98 &          0.66 &     -4.61 \\
  3w9e &    -9.93 &          -26.05 &         6.20 &   -22.64 & 13147.08 &            0.57 &      1136.57 &   625.69 &  3551.16 &          -13.75 &       213.27 &   103.55 &          38547.22 &                   -81.20 &              50193.13 &          27525.01 &          15845.44 &                   -74.70 &              41820.04 &          22926.32 &     277.09 &             -7.74 &          11.29 &      -1.53 &    143.46 &            -7.15 &          2.32 &     -5.87 \\
  4cmh &   -19.18 &          -19.86 &         6.02 &   -16.54 &  6897.76 &           -4.95 &        16.49 &     4.12 &  4984.19 &           -6.28 &       504.64 &   271.27 &          14825.35 &                   -19.34 &                773.01 &            405.82 &           3510.78 &                   -21.33 &               4521.46 &           2465.48 &     504.03 &             -3.17 &         341.51 &     184.67 &    145.62 &            -4.92 &          2.24 &     -3.69 \\
  4dtg &     6.29 &           -8.93 &         6.36 &    -5.43 &  8414.10 &          -24.78 &     27871.47 & 15304.52 &  2090.91 &           -0.98 &         0.00 &    -0.98 &          27043.45 &                    -4.79 &                276.62 &            147.35 &           1865.15 &                    -5.70 &               1700.42 &            929.53 &     111.13 &             -4.81 &          19.40 &       5.86 &     83.31 &            -7.64 &          4.29 &     -5.28 \\
  4dvr &    -6.74 &           -0.13 &         2.29 &     1.13 &  8488.06 &           -8.16 &        10.51 &    -2.38 &  1623.65 &           -2.40 &         0.28 &    -2.25 &           6163.79 &                   -18.24 &               4592.59 &           2507.68 &           1094.06 &                   -18.49 &               1535.07 &            825.80 &     139.59 &             -6.65 &           2.59 &      -5.22 &     53.45 &            -6.75 &          4.80 &     -4.11 \\
  4ffv &    28.69 &           -0.69 &         2.47 &     0.67 &  1711.64 &           -5.20 &         1.76 &    -4.23 &  1103.68 &           -3.79 &         0.78 &    -3.36 &            315.25 &                    -2.59 &                  0.15 &             -2.51 &           1730.40 &                    -2.52 &                  0.10 &             -2.46 &      70.33 &             -3.42 &           1.93 &      -2.36 &     40.20 &            -1.63 &          0.34 &     -1.44 \\
  4fqj &    33.50 &          -31.89 &        18.12 &   -21.93 & 11882.22 &           -5.03 &        37.25 &    15.46 &  2992.15 &           -4.56 &       113.49 &    57.86 &          40862.60 &                    -0.62 &                 69.22 &             37.46 &           9001.48 &                     1.95 &                 13.19 &              9.20 &     353.39 &             -5.71 &          33.95 &      12.96 &    617.51 &           -10.70 &          0.48 &    -10.44 \\
  4g6j &     0.30 &          -10.77 &         3.56 &    -8.81 &  7825.82 &            3.04 &        11.73 &     9.49 &  3134.64 &           -1.12 &       387.68 &   212.10 &           3000.58 &                    -2.68 &                704.39 &            384.73 &            585.45 &                    -8.83 &                961.45 &            519.97 &     128.27 &             -0.49 &           0.60 &      -0.16 &     67.11 &            -3.80 &          1.45 &     -3.00 \\
  4g6m &    -8.60 &          -23.53 &         3.48 &   -21.61 &  4350.90 &           -5.25 &         4.90 &    -2.56 &  2411.19 &           -2.85 &         1.89 &    -1.81 &           6731.08 &                   -25.68 &               9781.48 &           5354.13 &           2484.81 &                   -29.39 &               7116.34 &           3884.60 &      28.07 &             -6.08 &           1.57 &      -5.22 &      8.07 &            -6.45 &          0.44 &     -6.21 \\
  4h8w &    -1.33 &          -15.91 &         3.23 &   -14.14 &  9444.71 &           -5.18 &         4.61 &    -2.64 &  3646.47 &           -2.18 &         2.04 &    -1.05 &           2336.88 &                    -7.77 &                 11.57 &             -1.40 &            709.94 &                    -4.16 &                  0.35 &             -3.96 &     112.21 &             -6.52 &          12.46 &       0.33 &    131.44 &            -8.50 &          6.17 &     -5.11 \\
  4ki5 &    -8.15 &          -19.54 &         5.37 &   -16.58 &  2626.19 &           -3.59 &        56.69 &    27.58 &  4689.24 &           -1.58 &         0.00 &    -1.58 &          34867.78 &                    -8.27 &                  3.77 &             -6.20 &           2692.26 &                   -11.59 &                 39.94 &             10.37 &     166.79 &             -1.80 &           0.04 &      -1.78 &     76.98 &            -6.05 &          0.58 &     -5.73 \\
  4lvn &    40.37 &          -16.18 &         8.34 &   -11.59 &  4924.18 &            0.16 &       107.93 &    59.53 &  2298.31 &           -2.79 &         0.36 &    -2.59 &          27468.88 &                   -75.05 &              55150.31 &          30257.62 &          13994.77 &                   -57.50 &              42389.44 &          23256.70 &     504.98 &             -3.60 &           0.94 &      -3.09 &    177.60 &            -4.88 &          0.73 &     -4.48 \\
  4ot1 &   -13.23 &          -30.77 &         9.09 &   -25.77 &  3171.75 &           -3.07 &       186.61 &    99.56 & 12077.32 &           -2.27 &       846.11 &   463.09 &         123313.10 &                    -0.37 &                  0.00 &             -0.37 &          26002.74 &                     0.96 &                  9.39 &              6.12 &     178.79 &             -8.48 &          48.30 &      18.09 &    157.70 &            -4.40 &          0.01 &     -4.39 \\
  4qci &     5.68 &           -3.37 &         0.04 &    -3.35 &  1380.37 &            1.60 &       234.41 &   130.53 &  2333.97 &           -0.92 &         0.00 &    -0.92 &           6780.82 &                    -0.35 &                  0.00 &             -0.35 &            561.02 &                    -0.22 &                  0.00 &             -0.22 &      82.63 &             -2.29 &           0.04 &      -2.27 &     35.99 &            -2.01 &          0.16 &     -1.92 \\
  4xnq &   -18.37 &          -23.84 &         5.38 &   -20.88 &  9015.39 &           -5.83 &       132.70 &    67.16 &  4245.73 &          -11.41 &        56.38 &    19.60 &           9796.64 &                    -1.38 &                  0.06 &             -1.35 &           3476.40 &                    -2.27 &                  1.22 &             -1.60 &     282.80 &             -5.04 &           5.99 &      -1.74 &    117.00 &            -4.95 &          0.01 &     -4.94 \\
  4ydk &   -31.29 &          -38.30 &         7.69 &   -34.08 & 14702.85 &           -5.59 &         1.41 &    -4.81 & 11277.84 &          -12.23 &        56.62 &    18.91 &          62593.75 &                    -1.08 &                  0.00 &             -1.08 &          13719.03 &                    -2.36 &                  0.99 &             -1.82 &     593.74 &              5.84 &          31.03 &      22.91 &    915.51 &           -12.33 &          9.63 &     -7.04 \\
  5b8c &    -4.19 &          -21.12 &        10.70 &   -15.23 &  3181.60 &           -9.90 &        11.91 &    -3.35 &  2645.85 &           -5.77 &         0.53 &    -5.48 &          10337.48 &                    -8.24 &                  0.90 &             -7.74 &           1331.78 &                   -23.71 &               1650.60 &            884.12 &      56.26 &             -6.49 &           1.66 &      -5.57 &    118.91 &            -7.53 &          2.61 &     -6.09 \\
  5bv7 &    44.87 &          -39.40 &        38.47 &   -18.25 &  7939.79 &          -17.12 &       605.44 &   315.88 &  8220.14 &           -0.82 &         0.26 &    -0.67 &          58204.89 &                   -41.17 &              17180.44 &           9408.07 &          10666.16 &                   -27.71 &               3310.02 &           1792.80 &     214.86 &            -13.48 &          80.05 &      30.54 &    277.37 &            -5.08 &          3.23 &     -3.30 \\
  5d93 &    -6.28 &           -7.43 &         1.10 &    -6.83 &  7575.17 &           -4.57 &       269.76 &   143.80 &  1098.56 &           -6.74 &         3.11 &    -5.03 &           1735.32 &                   -13.51 &               3798.65 &           2075.75 &            844.67 &                    -8.86 &                  7.08 &             -4.97 &      48.56 &             -4.38 &           0.62 &      -4.04 &     64.57 &            -5.66 &          0.76 &     -5.25 \\
  5en2 &   -20.91 &          -12.80 &         5.68 &    -9.67 &  9216.24 &          -12.51 &      2053.41 &  1116.86 &  4036.15 &           -5.19 &         9.00 &    -0.23 &          42461.20 &                   -12.27 &                377.70 &            195.46 &           6825.12 &                   -26.61 &               1611.40 &            859.66 &     476.51 &            -10.44 &          35.10 &       8.86 &     87.25 &            -4.97 &          0.17 &     -4.87 \\
  5f9o &     5.96 &          -17.28 &         2.04 &   -16.16 &  4635.91 &            8.05 &       684.50 &   384.53 &  2466.22 &          -27.71 &       586.35 &   294.78 &          19935.98 &                    -4.91 &                 11.54 &              1.44 &           2840.79 &                   -10.34 &               2265.01 &           1235.41 &     147.07 &             -0.76 &           1.09 &      -0.17 &    168.54 &            -4.25 &          0.04 &     -4.22 \\
  5ggs &   -15.18 &          -21.95 &         7.63 &   -17.75 &  4550.44 &           -2.70 &        65.77 &    33.47 &  2931.98 &           -9.79 &        57.56 &    21.86 &          13470.10 &                    -0.50 &               1659.78 &            912.38 &           1195.70 &                   -10.36 &                894.55 &            481.64 &      94.70 &             -5.53 &           0.69 &      -5.15 &     71.94 &            -9.61 &          1.09 &     -9.01 \\
  5hi4 &     0.48 &          -20.27 &         4.00 &   -18.07 &  8816.86 &          -17.73 &     24243.98 & 13316.46 &  2147.64 &            3.02 &        14.51 &    11.00 &           2178.81 &                   -37.69 &               6188.73 &           3366.11 &           2011.06 &                   -31.65 &               6039.39 &           3290.01 &     108.56 &             -3.95 &           1.05 &      -3.37 &    152.57 &            -9.42 &          2.82 &     -7.87 \\
  5j13 &     0.61 &          -19.75 &         1.79 &   -18.76 &  9564.19 &           12.01 &      3451.90 &  1910.56 &  2439.57 &           -2.75 &         0.72 &    -2.35 &          23381.87 &                     0.01 &                 49.15 &             27.04 &           1690.91 &                    -3.15 &                  0.28 &             -3.00 &     106.87 &             -1.24 &           0.60 &      -0.91 &    140.27 &            -6.07 &          0.55 &     -5.77 \\
  5l6y &    -0.46 &          -12.26 &         3.31 &   -10.43 & 13722.44 &           -5.75 &       285.22 &   151.12 &  2982.89 &           -0.97 &         1.68 &    -0.05 &          22291.76 &                    -4.56 &                  3.86 &             -2.44 &           1380.57 &                    -4.34 &                  2.01 &             -3.24 &      64.99 &             -3.34 &           1.09 &      -2.75 &    194.99 &            -5.62 &          1.62 &     -4.73 \\
  5mes &   -16.95 &           -9.16 &         3.17 &    -7.42 &  7068.04 &           -2.95 &        68.05 &    34.47 &  1866.17 &           -5.79 &         1.48 &    -4.97 &           2680.68 &                    -1.74 &                  3.03 &             -0.07 &            423.94 &                    -2.18 &                  5.16 &              0.65 &     123.85 &             -7.40 &           0.96 &      -6.87 &     74.85 &           -12.49 &          3.20 &    -10.73 \\
  5nuz &   -18.37 &          -19.79 &         2.90 &   -18.19 & 11627.37 &           -2.92 &         1.29 &    -2.21 &  3260.21 &          -12.37 &        96.05 &    40.46 &          15824.23 &                   -53.72 &              14872.97 &           8126.42 &           5163.89 &                   -58.93 &               9124.02 &           4959.28 &     459.22 &            -14.15 &          89.50 &      35.07 &    120.05 &            -8.10 &          1.13 &     -7.48 \\
\bottomrule
\end{longtable}
% \renewcommand{\arraystretch}{1}
}







% \begin{longtable}{c|c|c}
%     \hline
%     Header 1 & Header 2 & Header 3 \\
%     \hline
%     \endfirsthead
%     \multicolumn{3}{|c|}%
%     {Table continues} \\
%         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\ 
%     \endhead
%     \hline
%             Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\ 
%             Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\         Entry 1111 & Entry 22222 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\ 
%     \multicolumn{3}{|r|}{Continued on next page} \\ \hline
%     \endfoot
%     Entry 1 & Entry 2 & Entry 3 \\ 
%     Entry 4 & Entry 5 & Entry 6 \\ 
%     ... & ... & ... \\ 
% \end{longtable}

==> tables/top1_success_rate.tex <==
\begin{tabular}{c|cccccccccc}
\toprule
       Method &    95\% &    90\% &   85\% &   80\% &   75\% &   70\% &   65\% &   60\% &   55\% &   50\%  \\
\midrule
    Reference & 100.00 & 100.00 & 94.55 & 92.73 & 90.91 & 87.27 & 76.36 & 70.91 & 60.00 & 60.00 \\
         HERN &   0.00 &   0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 \\
         MEAN &   0.00 &   0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 \\
       dyMEAN &   3.64 &   0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 \\
dyMEAN* &   1.82 &   0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 &  0.00 \\
       DiffAb &  56.36 &  23.64 & 18.18 & 14.55 & 10.91 &  3.64 &  0.00 &  0.00 &  0.00 &  0.00 \\
        AbDPO &  78.18 &  40.00 & 34.55 & 27.27 & 16.36 &  9.09 &  3.64 &  1.82 &  0.00 &  0.00 \\
\bottomrule
\end{tabular}
